Robustly Learning any Clusterable Mixture of Gaussians

We study the efficient learnability of high-dimensional Gaussian mixtures in the outlier-robust setting, where a small constant fraction of the data is adversarially corrupted. We resolve the polynomial learnability of this problem when the components are pairwise separated in total variation distance. Specifically, we provide an algorithm that, for any constant number of components $k$, runs in polynomial time and learns the components of an $\epsilon$-corrupted $k$-mixture within information theoretically near-optimal error of $\tilde{O}(\epsilon)$, under the assumption that the overlap between any pair of components $P_i, P_j$ (i.e., the quantity $1-TV(P_i, P_j)$) is bounded by $\mathrm{poly}(\epsilon)$. Our separation condition is the qualitatively weakest assumption under which accurate clustering of the samples is possible. In particular, it allows for components with arbitrary covariances and for components with identical means, as long as their covariances differ sufficiently. Ours is the first polynomial time algorithm for this problem, even for $k=2$. Our algorithm follows the Sum-of-Squares based proofs to algorithms approach. Our main technical contribution is a new robust identifiability proof of clusters from a Gaussian mixture, which can be captured by the constant-degree Sum of Squares proof system. The key ingredients of this proof are a novel use of SoS-certifiable anti-concentration and a new characterization of pairs of Gaussians with small (dimension-independent) overlap in terms of their parameter distance.

==> anticoncentration.tex <==
\section{Certifiable Anti-concentration}
\label[section]{sec:anticoncentration}

In this section, we prove \cref{lem:q-main}.
As in \cite{raghavendra2020list,karmalkar2019list}, we prove the lemma using tools from approximation theory.
For completeness we provide a proof from basic tools in approximation theory, following ideas from \cite{DGJ+:10}.

The starting point is the following elementary fact from approximation theory.

\begin{theorem}[Jackson's Theorem] \label[theorem]{thm:jacksons}
For every bounded continuous function $f \, : \, [-1,1] \rightarrow \R$ and every integer $\ell \geq 1$, 
there is a degree-$\ell$ polynomial $J$ such that
  \[
  \sup_{x \in [-1,1]} |J(x) - f(x)| \leq 6 \cdot \sup_{x,y \in [-1,1]} \{ |f(x) - f(y)| \, : \, |x-y| \leq \delta \}\mper
  \]
\end{theorem}

We will also need the following amplifying polynomial, as in \cite{DGJ+:10} -- the following fact follows from the Chernoff bound.

\begin{fact}[See \cite{DGJ+:10}, Claim 4.3]
  \label[fact]{fact:amplify}
  Let $k \geq 0$ be an even integer and let
  \[
  A_k(u) = \sum_{j \geq k/2} {k \choose j} \Paren{\frac{1+u}{2}}^j \Paren{\frac{1-u}{2}}^{k-j} \, .
  \]
  The degree-$k$ polynomial $A_k$ satisfies
  \begin{enumerate}
    \item if $u \in [3/5,1]$ then $A_k(u) \in [1-e^{-k/6}, 1]$, and
    \item if $u \in [-1,-3/5]$ then $A_k(u) \in [0,e^{-k/6}]$,
    \item if $u \in [-1,1]$ then $A_k(u) \in [0,1]$.
  \end{enumerate}
\end{fact}

We also need a bound on the rate of growth of univariate polynomials.

\begin{fact}[\cite{rivlin1974chebyshev}]
\label[fact]{fact:growth-bound}
  Let $a(t)$ be a polynomial of degree at most $d$ such that $|a(t)| \leq 1$ for all $t \in [-1,1]$.
  Then for all $t \geq 1$, $|a(t)| \leq |2t|^d$.
\end{fact}

Now we prove \cref{lem:q-main}.

\begin{proof}[Proof of \cref{lem:q-main}]
  Let $\delta > 0$ and let $f(x) \, : \, [-1,1] \rightarrow [0,1]$ be the following piecewise-linear function:
  \[
  f(x) = \begin{cases} 0, & |x| \geq 2\delta \\
                       (x+2\delta)/\delta, & -2\delta \leq x \leq -\delta \\
                       1, & |x|, \leq \delta\\
                       (-x+2\delta)/\delta, & \delta \leq x \leq 2\delta
          \end{cases} \, .
    \]
  The maximum slope of $0.9(f+0.1)$ is $1/\delta$.
  By \cref{thm:jacksons}, there is a degree-$100/\delta$ polynomial $J(x)$ 
  such that $|J(x) - 0.9(f(x)+0.1)| \leq 0.01$, for all $x \in [-1,1]$.
  Thus,
  \begin{enumerate}
  \item $J(x) \in [0,1]$ for all $x \in [-1,1]$.
  \item $J(x) \leq 0.2$ if $x \in [-1,-2\delta] \cup [2\delta,1]$.
  \item $J(x) \geq 0.8$ if $x \in [-\delta,\delta]$.
  \end{enumerate}

  For $k$ to be chosen later, let $A_k$ be as in \cref{fact:amplify}.
  Then the degree $d = 100k/\delta$ polynomial $A_k(J(x))$ satisfies
  \begin{enumerate}
  \item $A_k(J(x)) \in [0,1]$ for all $x \in [-1,1]$.
  \item $A_k(J(x)) \in [0,e^{-k/6}]$ if $x \in [-1,-2\delta] \cup [2\delta,1]$.
  \item $A_k(J(x)) \in [1,1-e^{-k/6}]$ if $|x| \leq \delta$.
  \item $|A_k(J(x))| \leq |2x|^d$ for all $|x| \geq 1$.
  \end{enumerate}
  We note that the last item follows from \cref{fact:growth-bound}.
  By construction, the same is true for $A_k(J(-x))$.

  For $L \geq 0$ to be chosen later, let
  \[
    p_{\delta,k,L}(x) = \Paren{\frac{A_k(J(x/L)) + A_k(J(-x/L))}{2}}^2\mper
  \]
  Then
  \begin{enumerate}
  \item $p_{\delta,k,L}(x) \in [0,1]$ for all $x \in [-L,L]$.
  \item $p_{\delta,k,L}(x) \in [0,e^{-k/6}]$ if $x \in [-L,-2\delta L] \cup [2\delta L, L]$.
  \item $p_{\delta,k,L}(x) \in [1,1-2e^{-k/6}]$ if $|x| \leq \delta L$.
  \item $|p_{\delta,k,L}(x)| \leq |2x/L|^{2d}$ for $|x| \geq L$.
  \item $p_{\delta,k,L}$ is even.
  \end{enumerate}

  Now we choose parameters in the following order.
  Let $k(\epsilon) = 6 \log(1/\e) + 1$ and let $L(\e) = (\log 1/e)^C / \e$ for $C > 0$ a sufficiently large constant.
  Let $\delta(\e) = \e/L(\e)$.
  Let $q_\e(x) = p_{\delta(\e),k(\e),L(\e)}(x)$.
  Then the following holds:
  \begin{enumerate}
  \item $q_\e(x) \in [0,1]$ for all $x \in [-L,L]$.
  \item $q_\e(x) \in [0,\e]$ if $x \in [-L,-2\e] \cup [2\e, L]$.
  \item $q_{\e}(x) \in [1,1-\e]$ if $|x| \leq \e$.
  \item $|q_{\e}(x)| \leq |2x|^{O((\log(1/\e)/\e^2))}$ for $|x| \geq L$.
  \item $q_{\e}$ is even.
  \end{enumerate}
  It just remains to verify that $\E_{x \sim \cN(0,1)} q_\epsilon(x) \leq O(\epsilon)$.
  We break up the expectation as
  \[
  \E_{x \sim \cN(0,1)} q_\e(x) \cdot (1_{|x| \leq \e} + 1_{|x| \in [\e,2\e]} + 1_{|x| \in [2\e,L]} + 1_{|x| \geq L})\mper
  \]
  The first three terms are all at most $O(\e)$ using our bounds above on $q_\e$.
  For the last term we have
  \[
  \E_{x \sim \cN(0,1)} q_\e(x) 1_{|x| \geq L} \leq \Pr(|x| \geq L)^{1/2} \cdot \Paren{ \E_{x \sim \cN(0,1)} (2x)^{O(\log(1/\e)/\e^2)}}^{1/2} \leq e^{-L^2/10} \cdot (\log(1/\e)/\e^2)^{O(\log(1/\e)/\e^2)}\mper
  \]
  Since $L^2 \geq (1/\e^2) (\log 1/\e)^C$ for sufficiently large $C$, this is at most $O(\e)$.
\end{proof}


==> constant-accuracy-old.tex <==
% !TEX root = writeup.tex

\section{Reduction to Constant-Accuracy Clustering and Proof of Main Theorem}
\label[section]{sec:constant-accuracy-and-main-theorem}

\Snote{TODO: put final putting-it-together here, I think}


\Snote{Daniel, please put constant-accuracy clustering lemma and proof here.}
In this section, we show how to recover a mixture that is close in total variation to the original mixture distribution, 
given a rough clustering of the samples.

Let the overlap of two distributions $P$ and $Q$ be $L(P,Q) = \int \min \{ dp,dq \}$. 
Note that this is $1-\dtv(P,Q)$. Let $h(P,Q) = -\log(L(P,Q))$. We will need the following lemma.
\begin{lemma}\label{largeOverlapLem}
Let $A$ and $B$ be two Gaussians with $h(A,B) = O(1)$. If $D \in \{ A, B\}$, then
\[ \Pr_{x \sim D} \left[1/\eps \geq  \frac{A(x)}{B(x)} \geq \eps \right] \geq 1- \poly(\eps) \;. \]
\end{lemma}
\begin{proof}
Without loss of generality, let $A$ be $\N(0, I)$ and take the probability measure with respect to $A$, i.e., $D = A$. 
The ratio $B(x)/A(x) = \exp(q(x))$ for some quadratic polynomial $q$. 
Since the overlap of $A$ and $B$ is large, $q$ must have constant $L_2$ norm with respect to $A$. 
The result then follows from Gaussian concentration for degree-$2$ polynomials.
\end{proof}

We will need a triangle inequality using ideas from~\cite{DKS17-sq}.

\begin{lemma}\label{triangleLem}
If $A,B,C$ are Gaussian distributions with $h(A,B)=O(1)$, then
\begin{equation}\label{eqn:hell_triangle}
h(A,C) = O(1 + h(B,C)) \;.
\end{equation}
\end{lemma}
\begin{proof}
From~\cite{DKS17-sq} it follows that for Gaussians $G$ and $H$ it holds
$h(G,H) = h_\Sigma(G,H)+h_\mu(G,H)$, 
where $h_\Sigma(G,H) = h(G',H')$ and $G'$, $H'$ are the mean $0$ translates of $G$ and $H$, respectively. 
By Proposition B.6 of that paper,
$$
h_\mu(G,H) = \inf_x ((x-\mu_G)\Sigma_G^{-1}(x-\mu_G)+(x-\mu_H)\Sigma_H^{-1}(x-\mu_H))/4 \;.
$$
From Proposition B.3 of that paper we have that
$$
h_\Sigma(A,C) = O(h_\Sigma(A,B)+h_\Sigma(B,C)) \;.
$$
Therefore, it suffices to prove that
$$
h_\mu(A,C) = O(1 + h_\mu(B,C)) \;.
$$
Note that we have
$$
h_\mu(B,C) = ((x-\mu_B)\Sigma_B^{-1}(x-\mu_B)+(x-\mu_C)\Sigma_C^{-1}(x-\mu_C))/4 \;,
$$
for some appropriately chosen $x$. Using that same value of $x$, we have that
$$
h_\mu(A,C) \leq ((x-\mu_A)\Sigma_A^{-1}(x-\mu_A)+(x-\mu_C)\Sigma_C^{-1}(x-\mu_C))/4 \;.
$$
The latter term is $O(h_\mu(B,C))$, while the former is $E=(x-\mu_A)\Sigma_A^{-1}(x-\mu_A)$. 
Since $h(A,B)=O(1)$, it is clear that $\Sigma_A=\Theta(\Sigma_B)$, 
and hence 
$$E=O((x-\mu_A)\Sigma_B^{-1}(x-\mu_A)) = O((x-\mu_B)\Sigma_B^{-1}(x-\mu_B)+(\mu_A-\mu_B)\Sigma_B^{-1}(\mu_A-\mu_B)) \;,$$
which is clearly $O(h_\mu(B,C)+1)$.
\end{proof}

\begin{proposition}\label[proposition]{prop:const-acc}
Let $X=\sum_{i=1}^k w_i G_i$ be a $k$-mixture of Gaussians with $h(G_i,G_j)$ at least a sufficiently large constant multiple of $\log(k/\eps)$ for all $i\neq j$. Let $X'$ be an $\eps$-corrupted version of $X$ and $N$ a sufficiently large polynomial in $nk/\eps$. 
Let $S$ be a set of $N$ random samples from $X'$. Let $T_1,\ldots,T_k\subset S$ be sets of samples so that, for some sufficiently small constant $c>0$, if $S_i$ is the set of samples in $S$ that were drawn from the $i$-th component of $X$ then $|T_i\cap S_i| \geq (1-c)\min(|T_i|,|S_i|)$ for all $i$. There exists an algorithm that given $S$, the $T_i$ and an additional set of $N$ independent samples from $X$, returns a list of Gaussians $H_1,\ldots,H_k$ so that $\sum_{i=1}^k w_i \dtv(H_i,G_i) \leq O(\eps\log(1/\eps))$ for all $i$.
\end{proposition}
\begin{proof}
First, we note that we can assume that $w_i\geq \eps/k$ for all $i$. 
The clusters with smaller weight can be identified with high probability by the size of the corresponding set $T_i$. 
The contribution to our sum of $w_i\dtv(H_i,G_i)$ from such clusters is $O(\eps)$, 
and treating all samples from such clusters as an additional source of error keeps the error rate at $O(\eps)$. 
We will assume this throughout the rest of the argument.

For each remaining cluster $T_i$, we note that $T_i$ has $1-c$ overlap with a large set of random samples from $G_i$. 
This means that it can be thought of as a set of independent samples from $G_i$ with a $c$-fraction of them adversarially corrupted. 
Applying the algorithm from~\cite{DKKLMS16} for robustly learning a single Gaussian to each component cluster, 
we can learn Gaussians $\tilde H_i$ so that, $\dtv(G_i,\tilde H_i) < 1/10$, and thus $h(G_i,\tilde H_i)=O(1)$.

Note that, by repeated applications of Lemma \ref{triangleLem}, this implies that 
for $i\neq j$ that $h(G_i, \tilde H_j)$ is at least a large multiple of $\log(k/\eps)$. 
This in turn implies that $\int \min(g_i(x),\tilde h_j(x))dx$ is a small polynomial in $\eps/k$, 
where $g_i(x)$ and $\tilde h_j(x)$ are the probability density functions of $G_i$ and $\tilde H_j$, respectively. 
This on the other hand is equal to
$$
\E_{x\sim G_i}[ \min(1,\tilde H_j(x)/G_i(x))] \;.
$$
This means that except with probability $(\eps/k)$ we have that $\tilde H_j(x)/G_i(x)$ is at most 
a small polynomial in $(\eps/k)$.

Given these $\tilde H_i$, we cluster the remaining $N$ samples in the following way. 
We associate each sample $x$ to the cluster $i$ for which the probability density function of $\tilde H_i(x)$ is largest. 
We claim that among the samples drawn from the component $G_i$, all but an $O(\eps/k)$-fraction of them end up in cluster $i$. 
This is because since $h(G_i,\tilde H_i)=O(1)$, Lemma \ref{largeOverlapLem} implies that for all but an $\eps/k$ fraction 
of these samples we have that $\tilde H_i(x)/G_i(x) > \poly(\eps/k)$. However, for all but an $\eps/k$-fraction 
of these samples we have that all other $\tilde H_j(x)/G_i(x)$ are less than a smaller polynomial in $\eps/k$.

Therefore, all but an $\eps/k$ fraction of samples from $G_i$ are assigned to the $i$-th cluster. 
Hence, among all $N$ samples, all but an $\eps$-fraction of them are non-corrupted 
samples that are assigned to the correct cluster. For each $i$, let $\eps_i$ be the fraction of samples 
assigned to the $i$-th cluster coming from other components 
or from errors plus the fraction of samples from the $i$-th component that were corrupted. 
It is easy to see that $\sum_{i=1}^k w_i\eps_i = O(\eps)$. Finally, running the robust estimation algorithm 
of \cite{DKKLMS16}, we can compute estimates $H_i$ so that $\dtv(H_i,G_i)=O(\eps_i \log(1/\eps_i))$ with high probability. 
Thus, the final error is $\sum w_i O(\eps_i \log(1/\eps_i))$, which is $O(\eps \log(1/\eps))$ 
by Jensen's inequality applied to the concave function $x\log(1/x)$.
\end{proof}


%\begin{theorem}\label{thm:main-thm}
%There is an algorithm which given an $\eps$-corrupted set of samples $X_1, \dots, X_n$ 
%drawn from a mixture of $d$-dimensional Gaussians $\sum_{i=1}^k w_i G_i$ with $w_i$ at least a sufficiently 
%large multiple of $\eps$ and such that for every $i\neq j$ the components $G_i$ and $G_j$ satisfy 
%$\dtv(G_i, G_j) \geq \max \{ 1-2^{-\min(w_i)^{-C}}, 1-\poly(\eps/k)\}$ and such that $\eps < 2^{-k^C}$ 
%and $n \geq d^{k^C}/\eps^C$ for $C$ a sufficiently large constant, the algorithm returns 
%Gaussians $H_1,\ldots,H_k$ so that for some permutation $\pi:[k]\rightarrow [k]$, 
%$\sum_{i=1}^k w_i\dtv(G_i,H_{\pi(i)}) = O(\eps\log(1/\eps))$ with probability $1-1/\poly(d)$. 
%The algorithm runs in time $n^{\poly(k)}$.
%\end{theorem}
\begin{proof}[Proof of \cref{thm:main-informal}]
In the case of uniform mixtures, our main theorem follows immediately by putting together \cref{lem:const_acc} and \cref{prop:const-acc}.
See \cref{sec:arbit-weights} for the case of nonuniform mixtures.
\end{proof}


==> covariance-separated.tex <==
\section{Covariance-Separated Case}

In this section we prove the following lemma. The setup for this section is as follows. Let $S_b$ denote the largest subset of $[k]$ such that every pair in $S_b$ is either mean, or variance separated. Let $S_g := \overline{S}_b$. 

\begin{lemma}
  \label[lemma]{lem:var-sep-main}
  Let $X_1,\ldots,X_n \in \R^d$ satisfy the $\delta,t$ deterministic conditions (\cref{def:deterministic}) with respect to Gaussians $G_1,\ldots,G_k$.
  Let $S_1,\ldots,S_k$ be the partition of $X_1,\ldots,X_n$ guaranteed by \cref{def:deterministic}.
  Let $Y_1,\ldots,Y_n$ be an $\e$-corruption of $X_1,\ldots,X_n$.
  For indeterminates $w_1,\ldots,w_n$, let $\alpha_i(w) = \sum_{j \in S_i} w_i$.
  For all $i,j \leq k$ and all unit $v \in \R^d$, the degree-$t$ the clustering axioms $\cA$ imply
 \begin{align}
 \cA \proves{O(1)} & O(1) \cdot \Paren{ (1/\eps_2) + \log(1/\eps_1)}  \cdot \frac{ \|\Sigma_{S_g}\|_2^{2} }{\|A\|_F^6}  + \frac{m_{a,b}}{\|A\|_F^8}\\
 &\geq \Paren{ 1-\frac{1}{n^4} \cdot O(\alpha_{S_g}^2(w) \alpha_{\overline{S_g}}^2(w))} \cdot \Paren{ (k/n)^8 \alpha_a(w)^8 - O(\xi^2) } \cdot \Paren{ (k/n)^8 \alpha_b(w)^8 - O(\xi^2) }
 \end{align}
  \Snote{statement in progress}
\end{lemma}
\begin{proof}
	For this proof, we will need the following claim.
	
	\begin{claim}~\label[claim]{claim:not_mean_not_var_cov_bound}
		If every pair $i,j \in S_g$ are neither $\eps_1$-mean separated, nor $\eps_2$-variance separated, then for every $j \in S_g$, 
		\[ \iprod{v,\Sigma_{S_g} v} \leq  O(1) \cdot \Paren{\frac{1 }{\eps_2} + \log \frac{1}{\eps_1}} \cdot \iprod{v, \Sigma_j v} . \]
	\end{claim}
	\begin{proof}	
		We know $\forall~i, j \in S_g$, for all $v \in \mathbb{R}^n$ 
		\begin{equation}~\label{eqn:not_mean_sep}
		|\iprod{ v, \mu_i - \mu_j}| \leq \frac{1}{10} \sqrt{\log \frac{1}{\eps_1}} \sqrt{\iprod{v, (\Sigma_i + \Sigma_j) v}} 
		\end{equation} 
		and 
		\begin{equation}~\label{eqn:not_var_sep}
		\max \{ \iprod{v,\Sigma_i v}, \iprod{v, \Sigma_j v} \} < \frac{\min \{ \iprod{v, \Sigma_i v}, \iprod{v, \Sigma_j v} \}}{\e_2}
		\end{equation} 
		Let $S := \cup_{i \in S_g} S_i$, $M :=(1/|S_g|) \cdot (\sum_{i \in S_g} G_i)$ and $\mu := \E_{x \sim M} [x]$. Then the covariance of the mixture is given by 
		\begin{align}
			\iprod{ v, \Sigma_{S_g} v} &= \sum_{i,j \in S} \iprod{X_i - X_j, v}^2 \\
			&\leq O(1) \cdot  \E_{x \sim M}\left[\iprod{ v, x-\mu}^2 \right] \\
			&= \frac{O(1)}{|S_g|} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu}^2 \right] \\ 
			&= \frac{O(1)}{|S_g|} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu_i + \mu_i - \mu}^2 \right] \\ 
			&\leq  \frac{O(1)}{|S_g|} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu_i}^2 + \iprod{v, \mu_i - \mu}^2 \right]  \\ 
			&=  \frac{O(1)}{|S_g|} \cdot \left( \sum_{i=1}^{|S_g|} \iprod{v, \Sigma_i v} + \iprod{v, \mu_i - \mu}^2 \right) \\
			&\leq O(1) \cdot \max_{i \in S_g} \Set{ \iprod{v, \Sigma_i v} } +  \frac{O(1)}{|S_g|} \cdot \left( \sum_{i=1}^{|S_g|} \iprod{v, \mu_i - \mu}^2 \right)
		\end{align}
		Applications of equations~\ref{eqn:not_var_sep} and~\ref{eqn:not_mean_sep} imply that for every $j \in [t]$ 
		\begin{align} 
			\iprod{ v,\Sigma_{S_g} v} &\leq \frac{\iprod{v, \Sigma_j v} }{\eps_2} + 4 \cdot \Paren{ \frac{1}{100} \cdot \log \frac{1}{\eps_1} \cdot \max_i \Set{ \iprod{v, \Sigma_i v} } }\\
			&\leq O(1) \cdot \Paren{\frac{1 }{\eps_2} + \log \frac{1}{\eps_1}} \cdot \iprod{v, \Sigma_j v} 
		\end{align}
		
	\end{proof}
	
The proof of our Lemma now follows from applications of~\cref{lem:fake_var_lowerbound} and \SKnote{6.5} . For any $a,b \in S_g$ let $p(x) := \iprod{x, (I - \Sigma_a^{-1/2} \Sigma_b \Sigma_a^{-1/2})x}$ and with $A = I - \Sigma_a^{-1/2} \Sigma_b \Sigma_a^{-1/2}$. The lemmas above imply 
		\begin{align}
	\cA \proves{O(1)} & \|\Sigma_{S_g}\|_2^{2} \|A\|_F^{2} \\
	&\geq \Paren{ 1-\frac{1}{n^2} \cdot O(\alpha_{S_g}(w) \alpha_{\overline{S_g}}(w))}^2 \cdot \Paren{ (k/n)^4 \alpha_a(w)^4 - O(\xi) }^2 \cdot \Paren{ (k/n)^4 \alpha_b(w)^4 - O(\xi) }^2 \\
	&\qquad \cdot \Paren{ \|A\|_F^4 - 2\cdot \log(1/\xi)^2 \cdot \|A\|_F^2 \cdot \Paren{ \|\Sigma_a\|_2 + \|\Sigma_b\|_2 }^2 }^2 \\
	&\qquad - (1-O(\alpha_{S_g}(w) \alpha_{\overline{S_g}}(w)))^2 \cdot m_{a,b}
	\end{align}
where $m_{a,b} := \eps^2 \cdot O(k^{20}) \cdot  \Paren{  (\Tr(A\Sigma_a ))^4  +  (\Tr(A\Sigma_b))^4 + (\Tr(A \Sigma(w)))^4 +  \iprod{\Sigma_a - \Sigma_b, A}^8 }$.\SKnote{This needs to be edited to reflect the new bounds}
Rearranging the above, and an application of \cref{claim:not_mean_not_var_cov_bound} and $x^2 - 2y^2 < 2(x-y)^2$ gives us 

\begin{align}
\cA \proves{O(1)} & O(1) \cdot \Paren{ (1/\eps_2) + \log(1/\eps_1)}  \cdot \frac{ \|\Sigma_{S_g}\|_2^{2} }{\|A\|_F^6}  + \frac{m_{a,b}}{\|A\|_F^8}\\
&\geq \Paren{ 1-\frac{1}{n^4} \cdot O(\alpha_{S_g}^2(w) \alpha_{\overline{S_g}}^2(w))} \cdot \Paren{ (k/n)^8 \alpha_a(w)^8 - O(\xi^2) } \cdot \Paren{ (k/n)^8 \alpha_b(w)^8 - O(\xi^2) }
\end{align}
	
%	\begin{claim}
%		For any $i \in S_g$ we have 
%		\[ \|\Sigma_{S_g}\| \leq \|\Sigma_i \| \]
%	\end{claim}
%	\begin{proof}
%		Recall $\Sigma_{S_g} := \frac{1}{n^2}\sum_{i,j} (X_i - X_j)^{\otimes 2}$. 
%	\end{proof}
	
\end{proof}


==> graveyard.tex <==

\subsection{OLD STUFF}

In this section we prove \cref{lem:constant-accuracy}.

%\Snote{TODO: write up proof of this from Daniel's email}

Let the overlap of two distributions $P$ and $Q$ be $L(P,Q) = \int \min \{ dp,dq \}$. Note that this is $1-TV(P,Q)$. Let $h(P,Q) = -log(L(P,Q))$. We will need the following lemma
\begin{lemma}
	Let $A$ and $B$ be two Gaussians with $h(A,B) = O(1)$. If $D \in \{ A, B\}$ then
	\[ \Pr_D \left[ \frac{A(x)}{B(x)} \geq \eps \right] \leq \poly(\eps). \]
\end{lemma}
\begin{proof}
	WLOG let $A$ be $\N(0, I)$ and take the probability measure wrt $A$. The ratio $B(x)/A(x) = \exp(q(x))$ for some quadratic polynomial $q$. Since the overlap of $A$ and $B$ is large, $q$ must have constant $L^2$ norm. The result then follows from Gaussian concentration for degree-2 polynomials.
\end{proof}

We use the following almost triangle inequality from [Ilias Daniel paper].
\begin{equation}\label{eqn:hell_triangle}
h(A,C) = O(h(A,B) + h(B,C)).
\end{equation}

First, run the algorithm from [robust regression] on $S_P$ and $S_Q$ to learn Gaussians $P'$ and $Q'$ with $h(P,P'), h(Q,Q') = O(1)$. An application of equation~\ref{eqn:hell_triangle} implies that the overlap between $P'$ and $Q'$ is still at most $\eps^{C'}$ for some large constant $C'$.

Our algorithm now again takes the samples and splits them into
buckets based on which of $P'$ or $Q'$ assigns larger likelihood. We claim that all but an $\eps$-fraction of the non-noisy points are classified correctly. This is because if the points were drawn from $P'$ and $Q'$, the probability of an error is exactly the overlap, $\eps^{C'}$. Consider the probability that a point drawn from $P$ gets misclassified as $Q'$. Let $S$ be the set of points that are classified as $Q'$. We note that $P'(S) < \eps^{C'}$. However, the set $T$ where $P(x)/P'(x) > \eps^{C'-1}$ has $P(T) < \eps$ by our Lemma (assuming $C'$ is large enough). So the probability $P(S)$ is at most $\left( P(T) + P'(S) \right)/\eps^{C'-1} = O(\eps)$. A similar argument holds for samples coming from $Q$.

Our algorithm now has sets of independent samples from $P$ and $Q$ with at most $\eps$ error and our standard Gaussian learning algorithm learns the mixture to error $\tilde{O}(\eps)$.


\section{Gauss facts}
 
\begin{lemma}\label{lem:gfact_1}
	If $x \sim \cN(a, \sigma)$, then 
	\[
	\E[x^4] - \E[x^2]^2 = 2 \sigma^4 + 4a^2 \sigma^2
	\]
\end{lemma}
\begin{proof}
	\begin{align*}
	\E[x^4] &= \E[(x-a + a)^4] = \E[(x-a)^4 + 4 (x-a)^3 a + 6 (x-a)^2 a^2 + 4 (x-a) a^3 + a^4] \\
	&= 3 \E[(x-a)^2]^2 + 6 a^2 \E[(x-a)^2] + a^4
	\end{align*}
	and 
	\begin{align*}
	\E[x^2]^2 &= \left( \E[(x-a)^2] + a^2 \right)^2 = \E[(x-a)^2]^2 + 2 \E[(x-a)^2] a^2 + a^4 
	\end{align*}
	Taking the differences gives us the lemma. 
\end{proof}

\begin{fact}[Basic facts]\label{fact:basic-fact}
	For any $a, b, c, d$ the following hold
	\begin{enumerate}
		\item 
		\begin{equation}
		\proves{k} (a+b)^k \leq 2^k \left(a^k + b^k\right)
		\end{equation}
		\item 
		\begin{equation}
		\left \{ (a-b)^{k} \leq t \right \} \proves{k} (a^2 - b^2)^{2k} \leq O_k \left( t^{2k} (t^{2k} + b^{2k}) \right) 
		\end{equation}
		\item 
		\begin{equation}
		\left \{ (a-b)^{k} \leq t, (c-d)^k \leq t \right \} \proves{k} (ac-bd)^k \leq O_k \left( t^{16} + t^8( d^8 + b^8) \right) 
		\end{equation}
	\end{enumerate}
\end{fact}
\begin{proof}
	for the final part
	For variables $a, b, c, d$, $(ac - bd)^8 = ((a-b+b)(c-d+d) - bd)^8 = ((a-b)(c-d) + (a-b)d + (c-d)b)^8 \leq O((a-b)^8(c-d)^8 + (a-b)^8d^8 + (c-d)^8b^8)$
\end{proof}


  \begin{claim}[Subsets to Population Moments]
  \label[claim]{clm:mom-2}
  \begin{equation}\label{eq:mom-3}
    \cA \proves{O(t)} \Paren{\sum_{i \leq n} w_i p(X_i) - \alpha_P(w) \E_{g \sim P} p(g) - \alpha_Q(w) \E_{g \sim Q} p(g)}^4 \leq O_t(\delta n^4 + \alpha_P(w) \alpha_Q(w)) \cdot \|p\|_\alpha^4 \mper
  \end{equation}
  \end{claim}
  \begin{proof}[Proof of \cref{clm:mom-2}]
  For later use, note that by \cref{def:deterministic,lem:emp-pop-2},
  \[
  \cA \proves{O(t)} \Paren{\sum_{i \in S_P} (p(X_i) - \E_{g \sim P}p(g) )}^2 \leq O_t(\delta) \cdot n^2 \cdot \|p\|^2
  \]
  and similarly for $Q$.
  Now,
  \[
  \sum_{i \in S_P} w_i p(X_i) - \alpha_P(w) \E_{g \sim P} p(g) = \sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)\mper
  \]
  By Cauchy-Schwarz,
  \[
  \cA \proves{O(t)} \Paren{\sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)}^2 \leq \alpha_P(w) \cdot \sum_{i \in S_P} w_i p(X_i)^2 + w_i \E_{g \sim P} p(g)^2\mper
  \]
  Using \cref{lem:emp-pop-2} and \cref{fact:hypercontractivity},
  \[
  \cA \proves{O(t)} \Paren{\sum_{i \in S_P} w_i p(X_i)^2}^2 \leq \alpha_P(w) \sum_{i \in S_P} p(X_i)^4 \leq O_t(\alpha_P(w)) \cdot n \cdot (\E_{g \sim P} p(g)^2 )^2
  \]
  and putting these together, we obtain
  \begin{equation}\label{eq:mom-3}
  \cA \proves{O(t)} \Paren{\sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)}^4 \leq O_t(\alpha_P(w))^3 \cdot n \cdot (\E_{g \sim P} p(g)^2)^2\mper
  \end{equation}
  In addition,
  \begin{align*}
  \cA  \proves{O(t)} & \Paren{\sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)}^2\\
  & = \Paren{\sum_{i \in S_P} (1-w_i) p(X_i) - \sum_{i \in S_P} (1-w_i) \E_{g \sim P} p(g) + |S_P| \E_{g \sim P} p(g) - \sum_{i \in S_P} p(X_i)}^2 \\
  & \leq O_t(\delta) \cdot n^2 \cdot \|p\|^2 + O_t(\alpha_Q(w)) \cdot \sum_{i \in S_P} (1-w_i)(p(X_i)^2 + \E_{g \sim P} p(g)^2)
  \end{align*}
  Here we used $\alpha_P(w) = n/2 - \alpha_Q(w)$.
  Following the same argument as for \eqref{eq:mom-3}, we obtain
  \[
    \cA \proves{O(t)} \Paren{\sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)}^4 \leq O_t(\alpha_Q(w))^3 \cdot n \cdot (\E_{g \sim P} p(g)^2)^2\mper
  \]
  Since for an indeterminate $u$ it is easy to show $\cA \cup \{ u \leq \alpha_Q(w)^3/n^3, u \leq \alpha_P(w)^3/n^3 \} \proves{O(1)}^{u,\cA} u \leq O(1/n^6) \cdot \alpha_P(w)^3 \alpha_Q(w)^3$, we have obtained
  \[
  \cA \proves{O(t)} \Paren{\sum_{i \in S_P} w_i p(X_i) - \sum_{i \in S_P} w_i \E_{g \sim P} p(g)}^4 \leq O_t(n^4 \cdot \delta) \|p\|^4 + \alpha_Q(w) \alpha_P(w) (\|p\|_\alpha^2)^2\mper
  \]
  Using a similar argument for $\sum_{i \in S_Q} w_i p(X_i) - \alpha_Q(w) \E_{g \sim P} p(g)$ finishes the claim.
  \end{proof}


We need the following lemmas for the covariance case``

\begin{lemma}~\label{lem:not_mean_not_var_cov_bound}\SKnote{Lemma for covariance separated case.}
	Let $M=\frac{1}{t} \left( G'_1 + \dots + G'_t\right)$ be a mixture of $t$ Gaussians with $G'_i := \cN(\mu_i, \Sigma_i)$. If every pair of Gaussians in this mixture are neither variance separated nor mean separated, then for any $i \in [t]$
	\[ \iprod{v, \cov(M)v} =  \left(\Paren{\log \frac{1}{\eps}} \cdot  \frac{1 }{\eps} \cdot \iprod{v, \Sigma_j v} \right)  \]
\end{lemma}
\begin{proof}	
	We know $\forall~i, j \in [t]$, for all $v \in \mathbb{R}^n$ 
	\begin{equation}~\label{eqn:not_mean_sep}
	|\iprod{ v, \mu_i - \mu_j}| \leq \frac{1}{10} \sqrt{\log \frac{1}{\eps}} \sqrt{\iprod{v, (\Sigma_i + \Sigma_j) v}} 
	\end{equation} 
	and 
	\begin{equation}~\label{eqn:not_var_sep}
	\max \{ \iprod{v,\Sigma_i v}, \iprod{v, \Sigma_j v} \} < \frac{\min \{ \iprod{v, \Sigma_i v}, \iprod{v, \Sigma_j v} \}}{\e}
	\end{equation} 
	Let The covariance of the mixture is given by 
	\begin{align}
	\iprod{ v, \cov(M)v} &= \E_{x \sim M}\left[\iprod{ v, x-\mu}^2 \right] \\
	&= \frac{1}{t} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu}^2 \right] \\ 
	&= \frac{1}{t} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu_i + \mu_i - \mu}^2 \right] \\ 
	&\leq  \frac{2}{t} \cdot \sum_i \E_{x \sim G_i} \left[ \iprod{ v, x-\mu_i}^2 + \iprod{v, \mu_i - \mu}^2 \right]  \\ 
	&=  \frac{2}{t} \cdot \left( \sum_{i=1}^t \iprod{v, \Sigma_i v} + \iprod{v, \mu_i - \mu}^2 \right) \\
	&\leq 2 \cdot \max_{i \in [t]} \Set{ \iprod{v, \Sigma_i v} } +  \frac{2}{t} \cdot \left( \sum_{i=1}^t \iprod{v, \mu_i - \mu}^2 \right)
	\end{align}
	Applications of equations~\ref{eqn:not_var_sep} and~\ref{eqn:not_mean_sep} imply that for every $j \in [t]$ 
	\begin{align} 
	\iprod{ v, \cov(M)v} &\leq \frac{\iprod{v, \Sigma_j v} }{\eps} + 4 \cdot \Paren{ \frac{1}{100} \cdot \log \frac{1}{\eps} \cdot \max_i \Set{ \iprod{v, \Sigma_i v} } }\\
	&\leq O\left(\Paren{\log \frac{1}{\eps}} \cdot  \frac{1 }{\eps} \cdot \iprod{v, \Sigma_j v} \right) 
	\end{align}
	
\end{proof}

In this case, we upper and lower bound the variance of a certain quadratic polynomial $p(X) := \iprod{X, (\Sigma_i - \Sigma_j) X}$ with respect to the fake gaussian. 

\begin{lemma}
	The polynomial $P(X) = \iprod{X, (\Sigma_i - \Sigma_j) X }$ satisfies 
	\begin{align}
		\Var_{\cN(\mu, \Sigma)}[P(X)] = 
	\end{align}
\end{lemma}
	\begin{align}
	\Norm{ \E_{X \sim G_i} [P(X)] -\E_{X \sim G_j} [P(X)] } &= \norm{ \Sigma_i - \Sigma_j }_F
	\end{align} 

\section{Removed from main-alg-analysis, april 13 at 2am}

We will prove the following main lemma about the algorithm \textsc{cluster}.

\begin{lemma}
\label[lemma]{lem:alphas-small}
  There is a constant $C \in \N$ such that for all $d$-dimensional Gaussians $G_1, \dots, G_k$ with $TV(G_a,G_b) \geq 1 - (\eta/k)$ for all $a, b \in [k]$, if $X_1,\ldots,X_n$ satisfy \cref{def:deterministic} with respect to $\{G_i \mid i \in [k]\}$ and $Y_1,\ldots,Y_n$ are an $\e$-corruption of $X_1,\ldots,X_n$ and $\{S_i \mid i \in [k]\}$ are the partition of $X_1,\ldots,X_n$ from \cref{def:deterministic}, then every degree $C$ pseudoexpectation which satisfies $\cA(Y_1,\ldots,Y_n,\e,\delta,C)$ has $\tfrac 1 {n^2} \pE \alpha_a(w) \alpha_b(w) \leq \delta^{\Omega(1)} + \e'(\e) + \eta'(\eta)$ for every $a, b \in [k]$ where $\lim_{\e \rightarrow 0} \e'(\e) = 0$ and $\lim_{\eta \rightarrow 0} \eta'(\eta) = 0$.
\end{lemma}
\SKnote{Edit to reflect right guarentees in the end. }

%\begin{lemma}[Main lemma on \textsc{cluster}]
%\label[lemma]{lem:main-cluster}
%  Let $\e > 0$ be sufficiently small, and let $X_1,\ldots,X_n \in \R^d$ satisfy the $t,\delta$ deterministic conditions with respect to Gaussians $P,Q$, for $\delta \leq \poly(\e/d)$, and suppose $Y_1,\ldots,Y_n$ are an $\e$-corruption of $X_1,\ldots,X_n$.
%  Then \textsc{cluster}$(Y_1,\ldots,Y_n,t,\e,\delta)$ returns a clustering with ??
%  \Snote{TODO: need to set parameters, in particular the value of $\delta$, here. The conclusion should be that as $t$ increases you get better and better error in the clustering that you output.}
%\end{lemma}
%


To finish the proof we rely on the following lemma, which says that a clustering with the guarantees we obtain by combining \cref{lem:round-analysis,lem:alphas-small} is enough to robustly learn a mixture of two Gaussians.
The proof, which we defer to \cref{sec:constant-accuracy}, relies on robust Gaussian learning algorithms from prior works.

\begin{lemma}
\label{lem:constant-accuracy}
\SKnote{Replace with Daniel's new lemma}
  There is a constant $C > 0$ such that for all small-enough $\e > 0$, there is an algorithm which takes
  \begin{compactenum}
  \item $n = \poly(d,1/\e)$ $\e$-corrupted samples from the mixture $\tfrac 1 2 (P + Q)$, where $P,Q$ are any Gaussian distributions on $\R^d$ with $TV(P,Q) \geq 1 - \e^C$, and
  \item a partition of those samples into two clusters $S_P, S_Q$ such that $|S_P \cap \{ \text{samples from P} \}| \geq (1/2 - 1/C)n$ and similarly for $S_Q$
  \end{compactenum}
  and with high probability returns $\widehat{\mu}_1,\widehat{\Sigma}_1, \widehat{\mu}_1, \widehat{\Sigma}_2$ such that $TV(\cN(\widehat{\mu}_1,\widehat{\Sigma}_1),A), TV(\cN(\widehat{\mu}_2,\widehat{\Sigma}_2), B) \leq \tO(\e)$.
  (Or the same with $1,2$ swapped.)
\end{lemma}

We can put together the lemmas to prove our main theorem.

\begin{proof}[Proof of \cref{thm:??}]
  \Snote{TODO: fill in proof}
  \SKnote{Done in COLT version -- needs editing for k-mix version}
\end{proof}

\subsection{Proof of \cref{lem:alphas-small}}

In this section we put together the proof of \cref{lem:alphas-small} from sub-lemmas which form the core of our SoS identifiability argument.
The following two sections will be devoted to these key identifiability lemmas.
We prove \cref{lem:alphas-small} in three cases; the cases are captured by the following lemma.

%\Snote{TODO: prove \cref{lem:gaussian-cases}, probably in appendix since this should be standard.}

\cref{lem:alphas-small} follows immediately from the following $4$ lemmas, which we prove in the next sections.

%KEEPING THE CLUSTERING LEMMA COMMENTED -- MIGHT NEED TO USE IT LATER THOUGH 
%\begin{lemma}[Clustering lemma]\label[lemma]{lem:cluster}
%	In the setting of \cref{lem:alphas-small}, defining for any polynomial $g$ the polynomial $\E_w [g(X)] := \frac{2}{n} \cdot \sum_{i \in [n]} w_i g(X_i)$, if there exists a polynomial $f : \mathbb{R}^d \rightarrow \mathbb R$ of degree $k$ satisfying 
%	\begin{enumerate}
%                \item $\E_{X \sim P} f(X) = 1$ and $\E_{V \sim Q} f(X) = -1$,
%		\item $\mathbb V_{Q}[f], \mathbb V_{P}[f] \leq \zeta$,
%		\item $\mathbb E_{Q} [ (f - \mathbb E_{Q} [f] )^4 ] \leq \zeta^2$ and similarly for $P$, and
%		\item $\cA \proves{} \E_w[(f(X) - \mu_f)^2] \leq \eta$ where $\mu_f = \tfrac k n \sum_{i \in [n]} w_i f(X_i)$
%	\end{enumerate}
%	then
%	\begin{align*}
%	\left( \frac{\alpha_P \alpha_Q}{n^2}\right)^{16} &\leq O_k \left(  (\zeta^8 + \eta^8 + (\eps + \delta)^2 \right)
%	\end{align*}
%%\end{lemma}
%
%\begin{lemma}[Mean-Separated SoS Identifiability]
%\label[lemma]{lem:mean-separated}
%  In the setting of \cref{lem:alphas-small}, if $P,Q$ are mean-separated (case 1 of \cref{lem:gaussian-cases}) then $f(X) = \tfrac{2}{\iprod{v,\mu_P - \mu_Q}} \cdot \iprod{v,X} - \tfrac{\iprod{v,\mu_P+\mu_Q}}{\iprod{v,\mu_P - \mu_Q}}$ satisfies the hypotheses of \cref{lem:cluster} with $\zeta,\eta \leq 1/(\log (1/\epsilon))^{\Omega(1)}$.
%\end{lemma}
%
%\begin{lemma}[Variance-Separated SoS Identifiability]
%\label[lemma]{lem:variance-separated}
%  In the setting of \cref{lem:alphas-small}, if $P,Q$ are variance-separated (case 2 of \cref{lem:gaussian-cases}) then there is a constant degree polynomial $f$, such that $f(\iprod{X, v})$ satisfies the hypotheses of \cref{lem:cluster} with what parameter settings?
%\end{lemma}
%
%\begin{lemma}[Covariance-Separated SoS Identifiability]
%\label[lemma]{lem:covariance-separated}
%  In the setting of \cref{lem:alphas-small}, if $P,Q$ are covariance-separated (case 3 of \cref{lem:gaussian-cases}), let
%  \[
%  Y = \Sigma_P^{-1/2} (X - (\mu_P + \mu_Q)/2)
%  \]
%  and
%  \[
%    g(X) = \frac{\iprod{Y, (I - \Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2}) Y}} {2\|I - \Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2}\|_F^2}
%  \]
%  then
%  \[
%  f(X) = g(X) - \E_P g(X) + 1
%  \]
%  satisfies the hypotheses of \cref{lem:cluster}
%   $\zeta,\eta \leq O(1/(\e^{-4}\|I-\Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2}\|)$.
%  \Snote{will need to do the trick here of passing to larger TV separation to kill this $1/\eps^4$.}
%\end{lemma}

\section{Removed from k-mix, april 13, 2:20am}

        \begin{align} 
         - O(1) \cdot \eps \cdot ( m_{a, b} + m_{a,a} + m_{b,b} ) \\
	&\qquad - O(1) \cdot \eps \cdot \iprod{v, \Sigma(w) v}^{4}
	\end{align}
	The final inequality follows from the fact that $\cA\proves{} w_iw_j\iprod{X_i' - X_j', v}^2 \geq 0$ for all $i, j$ and an application of \cref{lem:mom_decorruption_diff}.  We will need the following claim to continue. 
	\SKnote{Edit out probabilistic reasoning, shift to deterministic conditions. }
%HOEFFDING COMMENTED OUT
%	\begin{claim}\label[claim]{claim:restate_hoeffding}
%	Let $E$ be an event and $\cD$ be a distribution such that $\E_\cD [ 1_E(x)] = \xi$, then 
%	
%	\[ \Pr_{S \sim \cD^N}\Brac{ \sum_{x \in S} 1_E(x) \leq N \cdot (3\xi/2) } \geq \exp(-\Omega(\xi^2N)) \]  
%	\end{claim} 
%	\begin{proof}
%		This is just Hoeffding. 
%	\end{proof}
	\SKnote{Remove $d$ from degree and replace with $t$.}
	\begin{claim}\label[claim]{claim:gen_lower_bound}
		Let $f:(\R^{d})^2 \rightarrow \R$ be an arbitrary positive function,  $E \subseteq S_a \times S_b$ such that $f(X_i, X_j) \geq B$ and $|E| \geq (1-\xi)\cdot \Paren{\frac{n}{k}}^2$, then 
		\begin{align}
		\cA \proves{} \Brac{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j f(X_i, X_j)}^2 \geq \frac{B^2}{2} \cdot \Brac{ (k/n)^4  (\alpha_a(w) \alpha_b(w))^2 - O(\xi) \cdot (k/n)^2 \alpha_a(w) \alpha_b(w) }
		\end{align}
	\end{claim} 
	\begin{proof}
		
	
	\begin{align}
	\Brac{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j f(X_i, X_j)}^2 &\geq B^2 \cdot \Brac{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2\\
	&\geq \frac{B^2}{2} \cdot \Brac{ (k/n)^4  (\alpha_a(w) \alpha_b(w))^2 - \Theta(\xi) \cdot (k/n)^2 \alpha_a(w) \alpha_b(w) }
	\end{align}
	The final inequality follows from the following calculation  
	\begin{align} 
	(k/n)^4  (\alpha_a(w) \alpha_b(w))^2 &=  \Paren{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j) + \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{\bar{E}}(X_i, X_j) }^2 \\
	&\leq 2\Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2 + 2\Paren{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{\bar{E}}(X_i, X_j) }^2 \\ 
	&\leq 2\Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2 + (k/n)^2 \alpha_a(w) \alpha_b(w) O(\xi)
	\end{align} 
	Where the final inequality follows from Cauchy Schwartz. Rearranging, we get the claim. 
	\end{proof}
	
	We now apply \cref{claim:gen_lower_bound} with $f(x,y) := \iprod{x-y, v}^2$ and $E = E_a(v) \times E_b(v)$ where $E_a$ and $E_b$ are defined according to the deterministic conditions. Let $\Delta = \iprod{\mu_a - \mu_b, v}$ and $B = \Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^2$. 
	\begin{align}
	&\Brac{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j \iprod{ X_i - X_j, v}^2 }^2 \\
	&\geq \Omega(1) \cdot \Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 \\
	&\qquad \cdot \Brac{(k/n)^4   (\alpha_a(w) \alpha_b(w))^2 - \Theta(\xi) \cdot (k/n)^2 \cdot \alpha_a(w) \alpha_b(w) }
	\end{align}
	
	Similarly, an application of the same lemma with $E := F_a(v)$ (where $F_a(v)$ is defined in the deterministic condtions) implies
	
	\begin{align}
	&\Brac{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j \iprod{ X_i - X_j, v}^2 }^2 \geq \Omega(1) \cdot \Paren{\xi \cdot \iprod{v, \Sigma_a v} }^2 \cdot \Brac{ (k/n)^4  \alpha_a(w)^4 - \Theta(\xi) \cdot (k/n)^2 \alpha_a(w)^2 }
	\end{align}
	
	Substituting the terms above into equation~\ref{eqn:cov_lb_1} gives us 
	
	\begin{align}
	\cA \proves{} (2\iprod{v, \Sigma(w)v})^4 &= \Brac{\Paren{\frac{k}{n}}^{2} \sum_{i, j \leq n} w_i w_j \iprod{X_i'-X_j', v}^2}^4 \\
	&\geq \Brac{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j \iprod{X_i-X_j, v}^2}^4 \\
	&\qquad + \Brac{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a^{\otimes 2}} w_i w_j \iprod{X_i-X_j, v}^2 }^4 \\
	&\qquad + \Brac{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_b^{\otimes 2}} w_i w_j \iprod{X_i-X_j, v}^2 }^4 - O(1) \cdot \eps \cdot ( m_{a, b} + m_{a,a} + m_{b,b} )\\
	&\geq \Omega(1) \cdot \Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 \\
	&\qquad \cdot \Brac{(k/n)^4  (\alpha_a(w) \alpha_b(w))^2 - \Theta(\xi) \cdot (k/n)^2 \alpha_a(w) \alpha_b(w) }^2 \\
	&\qquad + \Omega(1 ) \cdot \Paren{\xi \cdot \iprod{v, \Sigma_a v} }^4 \cdot \Brac{ (k/n)^4 \alpha_a(w)^4 - \Theta(\xi) \cdot (k/n)^2 \alpha_a(w)^2 }^2 \\
	&\qquad + \Omega(1) \cdot \Paren{\xi \cdot \iprod{v, \Sigma_b v} }^4 \cdot \Brac{ (k/n)^4 \alpha_b(w)^4  - \Theta(\xi) \cdot (k/n)^2 \alpha_b(w)^2 }^2 \\
	&\qquad - O(1) \cdot \eps \cdot ( m_{a, b} + m_{a,a} + m_{b,b} )\\
	&\qquad - O(1) \cdot \eps \cdot \iprod{v, \Sigma(w) v}^{4}
	\end{align}

%	
%	This implies with probability $1-\delta$ for any $a \in [k]$,  $1-\xi$ of the samples drawn from $S_a$ satisfy $\iprod{X, v} = \iprod{\mu_a,v} \pm \sqrt{\log(1/\xi)} \cdot \sqrt{\iprod{v, \Sigma_a v}}$. Let $\Delta := \iprod{\mu_a - \mu_b, v}$ and $E$ denote the event where $	|X_i - \iprod{\mu_b, v}| \leq  \sqrt{\log(1/\xi)} \sqrt{\iprod{v, \Sigma_b v}}$ and $|X_i - \iprod{\mu_a,v}| \leq  \sqrt{\log(1/\xi)} \sqrt{\iprod{v, \Sigma_a v}}$
%	This means, 
%	\begin{align}
%	&\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j \iprod{X_i-X_j, v}^2 \\
%	&\geq \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)\Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^2 \\
%	&= \Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^2 \cdot \Brac{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}\\
%	&\geq \Paren{ \Delta - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^2 \cdot \Brac{ \alpha_a(w)^2 \alpha_b(w)^2 - \xi \alpha_a(w) \alpha_b(w) }
%	\end{align}
%	The final inequality follows from the following calculation  
%	\begin{align} 
%	\Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j}^2 &=  \Paren{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j) + \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{\bar{E}}(X_i, X_j)}^2 \\
%	&\leq 2\Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2 + 2\Paren{ \Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{\bar{E}}(X_i, X_j)}^2 \\ 
%	&\leq 2\Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2 + 2 \alpha_a(w) \alpha_b(w) \xi
%	\end{align} 
%	Where the final inequality follows from Cauchy Schwartz. Rearranging, we see 
%	\begin{align}
%	\alpha_a(w)^2 \alpha_b(w)^2  - 2 \xi  \alpha_a(w) \alpha_b(w) \leq \Paren{\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_b} w_i w_j 1_{E}(X_i, X_j)}^2
%	\end{align}
%	Let $E'$ denote the event 
%	
%	\begin{align} 
%	&\Paren{\frac{k}{n}}^{2} \sum_{(i, j) \in S_a \times S_a} w_i w_j \iprod{X_i-X_j, v}^2  \
%	&\geq \Brac{ \alpha_a(w)^2 \alpha_b(w)^2 - \xi \alpha_a(w) \alpha_b(w) }
%	\end{align} 
	
\end{proof}



==> k-mix.tex <==
% !TeX root    = writeup.tex

\section{Mixture of $k$ gaussians}
Let the original mixture of gaussians be given by $G_1,\dots, G_k$, let $C_i$ denote the subset of $X_1, \dots X_n$ drawn from $G_i$ and $\alpha_i(w) := \sum_{j \in C_i} w_i$. 
\begin{lemma} \Authornote{SK}{Edit}
	Let $\beta_{i, j}(w) := \sum_{S_i \cup S_j} w_i$. For any $i, j \in [k]$ if $i \neq j$, then 
	\[ \alpha_i(w) \alpha_j(w)  \leq  \epsilon \Paren{\frac{n}{k}}^2\]
\end{lemma}
\begin{proof}
	For any $a, b \in [k]$ if $G_a, G_b$ are mean separated, then the claim follows from \cref{lem:mean_sep}. If they are not mean separated and are variance separated, then the claim follows from \SKnote{refer right lemma}. 
	
	Let $I' \subset [n]$ be the largest set of indices such that for any pair of distinct $i, j \in I'$, $G_i, G_j$  are neither mean nor variance separated, but are covariance separated. Let $C$ denote the covariance of the mixture of clusters supported on $I'$. Since $i, j$ are covariance separated, there exists a polynomial $f_{i, j}$ satisfying the conditions in Lemma~\Authornote{SK}{Reference right lemma}, and so 
	\begin{equation}
	\Norm{ \E_{X \sim G_i}[P(X)] - \E_{X \sim G_j}[P(X)] } \geq \frac{\eps}{\log(1/\eps)} \cdot \Omega \Paren{ \norm{ (\Sigma_i - \Sigma_j) \cdot C }}
	\end{equation}
	Lemma~\ref{lem:not_mean_not_var_cov_bound} now implies the covariance of the mixture is at most $f(\eps) \Sigma_i$ for any $i$ \SKnote{Make this clearer as we go along.}
	
\end{proof}


\section{Mean-Separated Case}

\Snote{I think follwing proof can actually be omitted. It is just rearranging conclusions of variance bound lemmas.}
\begin{proof}[Proof of \cref{lem:mean_sep}]
Let $S_a, S_b$ denote samples corresponding to $G_a, G_b$
	

	\cref{lem:fake_var_lowerbound} implies, 
	\begin{align}
	\cA &\proves{O(1)} \iprod{v, \Sigma(w)v}^{4d} \\
	&\geq \Big[ \Omega(1) \cdot \Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 \label{eq:mean_sep_lb}\\
	&\qquad -O(\eps) \cdot   m_{a, b} \Big]^d \\
	&\qquad \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
	\end{align}
	An application of \cref{lem:fake_var_upperbound} implies 

	
\begin{align}
\cA &\proves{}  \iprod{v, \Sigma_a v}^{4d}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \iprod{v, \Sigma(w)v}^{4d} 
\end{align}

The above together imply 
\begin{align}
\cA &\proves{}  \iprod{v, \Sigma_a v}^{4d}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \\
&\qquad \cdot  \Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8\\
&\qquad - \eps \cdot  m_{a, b} \Big]^d \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
\end{align}
Rearranging these, we get
\begin{align}
\cA &\proves{}  \frac{\iprod{v, \Sigma_a v}^{4d}}{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^d}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
\end{align}
We repeat the above argument for $b$ to get 

\begin{align}
\cA &\proves{}  \frac{\iprod{v, \Sigma_b v}^{4d}}{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^d}\\
&\geq \exp(-O(d))\Brac{ (\alpha_b(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
\end{align}

Combining these, we get 

\begin{align}
\cA &\proves{}  \frac{\iprod{v, \Sigma_b v}^{8d} +\iprod{v, \Sigma_b v}^{8d} }{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^{2d}}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2\Brac{ (\alpha_b(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \\
&\qquad \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{4d}
\end{align}

%OLD STUFF	
%	\begin{align}
%\cA &\proves{} \eps \iprod{ v, \Sigma(w) v}^{16d} \\
%& \geq  \Paren{ \frac{k^2}{n^2} \sum_{i,j \in [n]} w_i w_j \iprod{v, \Sigma(w) v}^{8d}q_\eps \Paren{\frac{\iprod{X'_i - X'_j, v}}{\sqrt{\iprod{v, \Sigma(w)v}}}} }^2 \\
%& \geq \Paren{ \frac{k^2}{n^2} \sum_{i,j \in S_a} w_i w_j \iprod{v, \Sigma(w) v}^{8d}q_\eps \Paren{\frac{\iprod{X'_i - X'_j, v}}{\sqrt{\iprod{v, \Sigma(w)v}}}} }^2 \\
%& \geq \Paren{ \frac{k^2}{n^2} \sum_{i,j \in S_a} w_i w_j \Paren{\iprod{v, \Sigma(w) v}^{8d} - \frac{1}{2} \Paren{\frac{\iprod{X_i'-X_j',v}}{\eps}}^{16d}} }^2
%\end{align} 
%
%	Rearranging, we see 
%	\begin{align}
%	\cA \proves{} \eps \iprod{ v, \Sigma(w) v}^{16d} \geq \Paren{ \frac{\alpha_a(w)^2 k^2}{n^2} \iprod{v, \Sigma(w) v}^{8d} - \frac{k^2}{2 n^2 \epsilon^{2d}} \sum_{i, j \in S_a} w_i w_j \iprod{X_i'-X_j',v}^{16d}}^2
%	\end{align} 
%	
%	An application of \cref{lem:mom_decorruption_diff} with the $\eps$ parameter set to $2^{-1/\eps^4}$, and using the fact that $C(d) = \exp(\Omega(d))$ and $d = \log^C (1/\eps) \cdot 1/\eps^2$ implies 
%	\begin{align}
%	\Paren{ \frac{k^2}{n^2}\sum_{i, j \in S_a} w_i w_j \iprod{X_i'-X_j',v}^{16d} - \iprod{X_i - X_j, v}^{16d}}^2 &\leq C(16d) \cdot 2^{-1/\eps^4} \cdot \Paren{ \iprod{v, \Sigma_a v}^{8d} + \iprod{v,\Sigma(w) v}^{8d} } \\
%	&\leq  2^{-\Omega \Paren{1/\eps^4}} \cdot \Paren{ \iprod{v, \Sigma_a v}^{8d} + \iprod{v,\Sigma(w) v}^{8d} }
%	\end{align}	
%	\SKnote{incorporate edit above everywhere $\eps$ to $2^{-\Omega \Paren{1/\eps^4}}$.}
%	This implies 
%	\begin{align}
%	\cA &\proves{} \eps \iprod{ v, \Sigma(w) v}^{16d}\\
%	& \geq \Paren{ \Paren{ \frac{\alpha_a(w)^2 k^2}{n^2} - C(d) \cdot \eps }  \iprod{v, \Sigma(w) v}^{8d} - C(d) \eps \iprod{v, \Sigma_a v}^{8d} - \frac{k^2}{2 n^2 \epsilon^{16d}} \sum_{i, j \in S_a} w_i w_j \iprod{X_i-X_j,v}^{16d}}^2\\
%	&\geq \Paren{ \Paren{ \frac{\alpha_a(w)^2 k^2}{n^2} - C(d) \cdot \eps }  \iprod{v, \Sigma(w) v}^{8d} - (1 + \delta + \eps) \cdot C(d) \cdot \iprod{v, \Sigma_a v}^{8d}}^2
%	\end{align} 
%	Where the final inequality follows from concentration \SKnote{write, refer right lemma}.
%	An application of $\frac{1}{2}(a+b)^2 > a^2 + b^2$, and the fact that $\delta, \eps \leq 0.1$, now implies 
%	\begin{align}
%		\cA &\proves{} O\Paren{C(d) \iprod{v, \Sigma_a v}^{16d} } \geq
%		\Paren{ \frac{\alpha_a(w)^4 k^4}{n^4} - C(d) \cdot \eps  } \iprod{v, \Sigma(w) v}^{16d}  
%	\end{align} 
%	
%	  We now apply \cref{lem:var-lowerbound}, to get 
%	\begin{align}
%	\cA &\proves{} O\Paren{C(d) \iprod{v, \Sigma_a v}^{16d} } \\
%	&\geq 	\Paren{ \frac{\alpha_a(w)^4 k^4}{n^4} - C(d) \cdot \eps  } \cdot \Paren{ \cdot \frac{(k/n)^2 \alpha_a(w) \alpha_b(w)}{\eps^4} \cdot \iprod{ v, \Sigma_a v + \Sigma_b v}}^{16d}
%	\end{align} 
%	i.e. 
%	\begin{align}
%	\cA \proves{} \Paren{ (k/n)^4 \alpha_a(w)^4  - C(d) \cdot \eps  } \cdot \Paren{(k/n)^2 \alpha_a(w) \alpha_b(w)}^{16d} &\leq  \epsilon^{64d} \cdot O\Paren{ C(d) } \cdot \Paren{\frac{\iprod{v, \Sigma_a v}}{ \iprod{ v,\Sigma_a v+\Sigma_b v}} }^{16d} \\
%	&\leq \epsilon^{64d} \cdot O\Paren{ C(d) }
%	\end{align} 
%	Since $d = (\log 1/\eps)^C \cdot 1/\eps^2$, this translates to
%	\begin{align}
%	\cA &\proves{} \Paren{ (k/n)^4 \alpha_a(w)^4  - \exp ((\log 1/\eps)^C \cdot 1/\eps^2) \cdot \eps  } \cdot \Paren{(k/n)^2 \alpha_a(w) \alpha_b(w)}^{16 \cdot (\log 1/\eps)^C \cdot 1/\eps^2}\\
%	&\leq \exp \Paren{ -64 \cdot (\log 1/\eps)^{C+1} \cdot 1/\eps^2  + (\log 1/\eps)^C \cdot 1/\eps^2 }\\
%	&\leq \exp \Paren{ \Omega \Paren{- (\log 1/\eps)^{C+1} \cdot 1/\eps^2}}
%	\end{align} 

\end{proof}



==> lemma-cluster.tex <==
\section{Clustering lemma}

In this section, we prove \cref{lem:cluster}. Let $q_f(X) := (f(X) - \E_P[f])^2 (f(X) - \E_Q[f])^2$. We give upper and lower bounds on the quantity $\E_w[q_f(X)]$. 

We first prove the upper bound. Since $w_i^2 = w_i$ we have $w_i \leq 1$ and $q_f(X'_i) \geq 0$ for ghost samples $X'_i$, 
\begin{equation}
\cA \proves{} \E_w[q_f(X')]^8 \leq \left( \frac{2}{n} \sum_i q_f(X'_i) \right)^8.
\end{equation}

There is a degree 2 sum-of-squares proof of $(a+b)^8 \leq O(a^8 + b^8)$. This implies 
\begin{equation}
\cA \proves{} \E_w[q_f(X')]^8 \leq O\left( \left( \frac{2}{n} \sum_i q_f(X'_i) - \E_{P/2 +Q/2}[q_f(X)] \right)^8 +  \E_{P/2 +Q/2}[q_f(X)]^8 \right).
\end{equation}
An application of Lemma~\ref{lem:moment-compare} now implies 
\begin{equation}
\cA \proves{}  \left( \frac{2}{n} \sum_i q_f(X'_i) - \E_{P/2 +Q/2}[q_f(X)] \right)^8 \leq O_k\Paren{\e + \delta} \|q_f\|^8 + \Var_{P, Q}[q_f]^4
\end{equation}
Since $\|q_f\|^8 = \frac{1}{2}\left( \E_{P} [q^2_f(X)]^4 + \E_Q [q^2(X)]^4 \right)$. An application of hypercontractivity (Fact~\ref{fact:hypercontractivity}) and using the fact that $q_f$ is a square polynomial, now gives us 
\begin{equation} 
\|q_f\|^8 \leq O_k \left( \left( \E_{P} [q_f(X)]^8 + \E_Q [q(X)]^8 \right) \right) \leq O_k \left( \E_{P/2 +Q/2}[q_f(X)]^8 \right). 
\end{equation} 
Additionally $\Var_{P, Q}[q_f] = \frac{1}{2} \E_P[(q_f(X) - \E_P[q_f(X)])^2] + \frac{1}{2} \E_Q[(q_f(X) - \E_Q[q_f(X)])^2]$. Further applications of hypercontractivity and $(a+b)^2 \leq O(a^2 + b^2)$ show $\Var_{P, Q}[q_f]  \leq O\left( \E_{P/2 +Q/2}[q_f(X)]^2 \right)$. This implies,
\begin{equation}
\cA \proves{} \left( \frac{2}{n} \sum_i q_f(X'_i) - \E_{P/2 +Q/2}[q_f(X)] \right)^8 +  \E_{P/2 +Q/2}[q_f(X)]^8 \leq O_k \left( \E_{P/2 +Q/2}[q_f(X)]^8 \right) 
\end{equation}
Since $\proves{} \E_P[g(X) h(X)]^2 \leq \E_P[g(X)^2] \E_P[h(X)^2]$ has a degree 2 sum-of-squares proof, we see 
\begin{align}
\cA &\proves{} \E_{P/2 +Q/2}[q_f(X)]^8 = \E_{P/2 + Q/2}[(f(X) - \E_P[f])^2 (f(X) - \E_Q[f])^2]^8 \\
&= \frac{1}{2} \sum_{T \in \{P, Q\}} \E_T \left[(f(X) - \E_P[f])^2 (f(X) - \E_Q[f])^2 \right]^8 \\ 
&\leq \frac{1}{2} \sum_{T \in \{P, Q\}} \E_T \left[ (f(X) - \E_P[f])^4 \right]^4 \E_T \left[ (f(X) - \E_Q[f])^4 \right]^4
\end{align}
We now analyze each term in the above sum. Since $P$ is hypercontractive, applying Fact~\ref{fact:hypercontractivity}, we see
\begin{align}
\proves{} \E_P \left[ (f(X) - \E_P[f])^4 \right]^4 \E_P \left[ (f(X) - \E_Q[f])^4 \right]^4 \leq \Var_P[f]^8 \E_P \left[ (f(X) - \E_Q[f])^4 \right]^4
\end{align}
Adding and subtracting $\E_P[f]$ for the term on the right hand side, and using Fact~\ref{fact:basic-fact} we get 
\begin{align}\label{eqn:prefinal}
\proves{} \E_P \left[ (f(X) - \E_Q[f])^4 \right]^4 \leq \Var_P[f]^8 + (\E_P[f] - \E_Q[f])^{16}
\end{align}
Substituting these back in, we see 
\begin{align} 
\cA \proves{} \E_{P/2 +Q/2}[q_f(X)]^8 &\leq \Var_P[f]^{16} + \Var_Q[f]^{16} + (\Var_P[f]^8 + \Var_Q[f]^8)(\E_P[f] - \E_Q[f])^{16}
\end{align}
From the conditions of the theorem, we have $\cA \proves{} \Var_P[f]^{k} \leq \zeta^{k} (\E_P[f] - \E_Q[f])^{2k}$. Putting everything together, we get an upper bound on $\E_w[q_f(X')]^8$. 
\begin{align} \label{eqn:upper}
\cA \proves{} \E_w[q_f(X')]^8 &\leq O_k \left( (\zeta^{16} + \zeta^8) (\E_P[f] - \E_Q[f])^{32} \right)
\end{align}


To prove the lower bound, observe that $(f(X) -\E_P[f]) - \frac{\alpha_Q}{n} (\E_Q[f] - \E_P[f]) = f(X) - \E_w[f] + \E_w[f] - \E_{\alpha_P P + \alpha_Q Q}[f]$. Using Lemma~\ref{lem:moment-compare} and Fact~\ref{fact:basic-fact} as before, we get 
\begin{align*}
\cA \proves{} \left( (f(X) -\E_P[f]) - \frac{\alpha_Q}{n} (\E_Q[f] - \E_P[f]) \right)^8 \leq O_k \left( \left(f(X) - \E_w[f]\right)^8 + (\eps + \delta) \|f\|^8 + \Var_{P,Q}[f]^4 \right)
\end{align*}
Let the right hand side above be denoted by $\Delta(X)$. Then an application of Fact~\ref{fact:basic-fact} gives us 
\begin{align*}
\cA \proves{}& \left((f(X) -\E_P[f])^2 - \frac{\alpha_Q^2}{n^2}(\E_Q[f] - \E_P[f])^2 \right)^8  \leq O\left(  \Delta(X) \cdot \left( \Delta(X) + \frac{\alpha_Q}{n}^8  (\E_Q[f] - \E_P[f])^8 \right) \right) 
\end{align*}
A similar inequality holds for $Q$ as well. Applying Fact~\ref{fact:basic-fact} to $(f(X) -\E_P[f])^2$, $\frac{\alpha_Q^2}{n^2}(\E_Q[f] - \E_P[f])^2$ and the corresponding terms for $Q$ we see
\begin{align*}
\cA \proves{} & \left(\E_w[q_f(X) - \frac{\alpha_P^2 \alpha_Q^2}{n^4} (\E_P[f] - \E_Q[f])^2 (\E_Q[f] - \E_P[f])^2 ]\right)^8 \leq O \left( \E_w \left[ \Delta^4 + \Delta^2 \cdot (\E_P[f] - \E_Q[f])^{16}  \right] \right)\\
& \leq O_k \left( \E_w \left[\left(f(X) - \E_w[f]\right)^2 \right]^{16} + (\eps + \delta)^4 \|f\|^{32} + \Var_{P, Q}[f]^{16} \right) \\
& +~O_k \left( \E_w \left[\left(f(X) - \E_w[f]\right)^2 \right]^8 +  (\eps + \delta)^2 \|f\|^{16} + \Var_{P, Q}[f]^8 \right) (\E_P[f] - \E_Q[f])^{16}
\end{align*}
Since $f$ is normalized s.t. $\E_Q[f] = 1$ and $\E_P[f] = -1$ 
\[\|f\|^2 = \E_{P/2 + Q/2}[f^2(X)] = \Var_P[f] + \Var_Q[f] + O\left( \E_P[f]^2 + \E_Q[f]^2 \right) \leq \Var_P[f] + \Var_Q[f] + O\left( \E_P[f] - \E_Q[f] \right)^2.\]
Substituting this back in, and using the fact that $\cA \proves{} \E_w[(f-\mu_f)^2] \leq \eta \cdot \left( \E_P[f] - \E_Q[f] \right)^2$ and $\Var_{P, Q}[f] \leq \zeta \cdot \left( \E_P[f] - \E_Q[f] \right)^2$, we get 
\begin{equation}\label{eqn:diff}
\cA \proves{} \E_w \left[q_f(X) - \frac{\alpha_P^2 \alpha_Q^2}{n^4} (\E_Q[f] - \E_P[f])^4 \right]^8 \leq O_k \left( \eta^8 + (\eps + \delta)^2 + \zeta^8 \right) \cdot \left( \E_P[f] - \E_Q[f] \right)^{32}
\end{equation}

We upper bound $\frac{\alpha_P^2 \alpha_Q^2}{n^4} (\E_P[f] - \E_Q[f])^4$ in terms of $\E_w[q_f(X)]$, by adding and subtracting $q_f(X)$. 
\begin{align*} 
\cA \proves{} \E_w \left[\frac{\alpha_P^2 \alpha_Q^2}{n^4}(\E_P[f] - \E_Q[f])^4\right]^8
\leq C \cdot \left( \E_w[q_f(X)]^8 + \E_w \left[\frac{\alpha_P^2 \alpha_Q^2}{n^4} (\E_P[f] - \E_Q[f])^4 - q_f(X)\right]^8 \right)
\end{align*} 
For some constant $C$. Rearranging the above inequality, we get that $\cA$ proves 
\begin{equation}
C \cdot \E_w[q_f(X)]^8  \geq \left(\frac{\alpha_P \alpha_Q}{n^2}\right)^{16} (\E_P[f] - \E_Q[f])^{32} - C \E_w \left[ \frac{\alpha_P^2 \alpha_Q^2}{n^4} (\E_P[f] - \E_Q[f])^4 - q_f(X) \right]^8 
\end{equation}
Equations~\ref{eqn:upper} and~\ref{eqn:diff} now give us
\begin{align*}
\left( \frac{\alpha_P \alpha_Q}{n^2}\right)^{16} &\leq O_k \left(  (\zeta^8 + \eta^8 + (\eps + \delta)^2 \right)
\end{align*}
Where we used the fact that $\zeta < 1$. 


==> mean-separation.tex <==
\section{Robust Identifiability: Separated Means}
In this section we prove \cref{lem:mean-separated}.
We start with some notation.
For Gaussians $P,Q$ satisfying the mean separation condition with unit vector $v$, we define a polynomial in variables $x = (x_1,\ldots,x_d)$ with coefficients depending on the indeterminates of $\cA$ by
\[
q(x) = (\iprod{x - \mu(w), v} - \iprod{\mu_P - \mu(w),v})(\iprod{x - \mu(w), v} - \iprod{\mu_Q - \mu(w),v})\mper
\]
Note that $q(x) = 0$ iff $\iprod{x,v} = \iprod{\mu_P,v}$ or $\iprod{x,v} = \iprod{\mu_Q,v}$.

We also define $\mu_\alpha(w) = 2 \alpha_P(w) \mu_P/ n + 2 \alpha_Q(w) \mu_Q / n$.

The main idea will be that the $2$nd moment of $q$ under the empirical distribution of a subset of half the samples is too large unless that subset of samples is actually one of the correct clusters.
Our first lemma on the way to \cref{lem:mean-separated} says that the empirical distribution of $q$ evaluated on a subset of samples with Gaussian moments has lower-bounded second moment.

\begin{lemma}
  \label[lemma]{lem:q-2nd-moment}
  As a polynomial in $w$,
  \[
  \E_{x \sim \cN(0,\Sigma(w))} q(x)^2 \succeq 3 (\E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2)^2 - (\iprod{\mu_P,v} - \iprod{\mu_Q,v})^2 \cdot \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2\mper
  \]
\end{lemma}

The second lemma will allow us to upper bound the left-hand side of the expression in \cref{lem:q-2nd-moment}.

\begin{lemma}
  \label[lemma]{lem:q-upper}
  If $\pE$ satisfies $\cA$ and $P,Q$ have TV distance at least $1/2$ 
  \[
  \pE \E_{x \sim \cN(0,\Sigma(w))} q(x)^2 \leq \text{ something $ \ll \iprod{\mu_P - \mu_Q,v}^4$ here}
  \]
  \Snote{TODO: finish stating this lemma, use it to complete the proof of \cref{lem:mean-separated}}.
\end{lemma}

The next lemma is a straightforward calculation.

\begin{lemma}
  \label[lemma]{lem:mean-sep-1}
  Under the mean separation condition of \cref{lem:mean-separated} if $TV(P,Q) \geq 1 - \eta$, then
  \begin{align*}
  \cA \proves{O(1)}  \E_{g \sim 2 \alpha_P(w) P /n + 2 \alpha_Q(w) Q /n} & \iprod{g - \mu_\alpha(w),v}^2 \\
  & \geq \Brac{\frac 1 {n^2} \cdot O(\alpha_P(w) \alpha_Q(w)) + \eta^{\Omega(1)}} \cdot \iprod{\mu_P - \mu_Q,v}^2 \mper
  \end{align*}
\end{lemma}

Finally we will need the following to control error terms:
\begin{lemma}
  \label[lemma]{lem:p-norm-bounds}
  Let $p(x)= \iprod{x - \mu_\alpha, v}^2$.
  Suppose the mean separation condition holds for $P,Q$ with total variation distance at least $1 - \eta$.
  Then
  \[
  \cA \proves{O(1)} \|p\|^2 \leq O(\iprod{\mu_P - \mu_Q,v})^4 \qquad \cA \proves{O(1)} \|p\|_\alpha^2 \leq O(\alpha_P(w)^2 \alpha_Q(w)^2/n^4 + \eta^{\Omega(1)}) \iprod{\mu_P - \mu_Q,v}^4\mper
  \]
  Let $r(x) = \iprod{x - \mu_\alpha,v}$.
  Then
  \[
  \cA \proves{O(1)} \|r\|^2 \leq O(\iprod{\mu_P - \mu_Q,v}^2) \qquad \cA \proves{O(1)} \|p\|_\alpha^2 \leq O(\alpha_P(w) \alpha_Q(w)/n^2 + \eta^{\Omega(1)}) \iprod{\mu_P - \mu_Q,v}^2\mper
  \]
\end{lemma}

Now we can prove \cref{lem:mean-separated}.

\begin{proof}[Proof of \cref{lem:mean-separated}]
  Suppose $X_1,\ldots,X_n$ satisfy \cref{def:deterministic} with respect to $P,Q$ for $\delta > 0$ and $t = 100$.
  Let $\pE$ of degree $100$ satisfy $\cA$.
  We can bound $\pE \alpha_P(w) \alpha_Q(w)$ as follows:
  \begin{align*}
  & \frac 1 {n^2} \pE \alpha_P(w) \alpha_Q(w)\\
  & \leq \frac {\pE \E_{g \sim 2 \alpha_P(w) P/n + 2 \alpha_Q(w) Q/n} \iprod{g - \mu_\alpha(w),v}^2}{\iprod{\mu_P - \mu_Q,v}^2} + \eta^{\Omega(1)} \text{ by \cref{lem:mean-sep-1}}\\
  & \leq \frac {\pE \frac 2 n \sum_{i \leq n} w_i \iprod{X_i' - \mu_\alpha(w),v}^2 + O\Paren{\pE (\e +\delta) \|p\|^8 + \pE \alpha_P(w) \alpha_Q(w)/n^2 \cdot \|p\|_\alpha^8}^{1/8}}{\iprod{\mu_P - \mu_Q,v}^2}  + \eta^{\Omega(1)} \\
  & \qquad \text{ by \cref{lem:moment-compare}, where $p(x) = \iprod{x - \mu_\alpha(w),v}^2$}\\
  &  \leq \frac {\pE \E_{g \sim \cN(\mu(w),\Sigma(w))} \iprod{g - \mu_\alpha(w),v}^2 + O\Paren{\pE (\e +\delta) \|p\|^8 + \pE (\alpha_P(w) \alpha_Q(w) / n^2) \|p\|_\alpha^8}^{1/8}}{\iprod{\mu_P - \mu_Q,v}^2}  + \eta^{\Omega(1)} \\
  & \qquad \text{ by \cref{lem:emp-pop}, folding errors into the $O(\delta) \pE \|p\|^8$ term }\\
  & \leq \frac{\pE \E_{g \sim \cN(\mu(w),\Sigma(w))} \iprod{g - \mu_\alpha(w),v}^2}{\iprod{\mu_P - \mu_Q,v}^2} + (\e + \delta)^{\Omega(1)} + O (\pE (\alpha_P(w) \alpha_Q(w) / n^2)^9)^{1/8} + \eta^{\Omega(1)}\\
  & \qquad \text{ by \cref{lem:p-norm-bounds}.}
  \end{align*}
  Now,
  \[
  \E_{g \sim \cN(\mu(w),\Sigma(w))} \iprod{g - \mu_\alpha(w),v}^2 = \E_{g \sim \cN(0,\Sigma(w))} \iprod{g + \mu(w) - \mu_\alpha(w),v}^2 = \E_{g \sim \cN(0,\Sigma(w))} \iprod{g,v}^2 + \iprod{\mu(w) - \mu_\alpha(w),v}^2
  \]
  By \cref{lem:moment-compare} and \cref{lem:p-norm-bounds},
  \begin{align*}
  & \pE \E_{g \sim \cN(\mu(w),\Sigma(w))} \iprod{g - \mu_\alpha(w),v}^2 \\
  & \leq \pE \E_{g \sim \cN(0,\Sigma(w))} \iprod{g,v}^2 + (\e + \delta)^{\Omega(1)} \iprod{\mu_P - \mu_Q,v}^2 + (\pE( \alpha_P(w) \alpha_Q(w) / n^2)^9)^{1/8} \iprod{\mu_P - \mu_Q,v}^2\mper
  \end{align*}
  \Snote{TODO: fill in the rest of this proof as follows. First use \cref{lem:q-2nd-moment} to get to $\E_{x \sim \cN(0,\Sigma(w))} q(x)^2$. Then go from population to ghost samples $X_i'$, and then to the "ideal" mixture via \cref{lem:moment-compare} (this logic can be contained in \cref{lem:q-upper}). Under the ideal mixture, should get a bound which is $\ll \iprod{\mu_P - \mu_Q, v}^2$ on $\pE \E_{g \sim \cN(\mu(w),\Sigma(w))} \iprod{g - \mu_\alpha(w), v}^2$. This allows us to conclude that $n^{-2} \pE \alpha_P(w) \alpha_Q(w) \leq \text{small} + O(\pE \alpha_P(w)^9 \alpha_Q(w)^9 / n^{18})^{1/8}$. Last step is to apply some lemma (which should go in the appendix) saying that this implies $\pE \alpha_P(w) \alpha_Q(w) / n^2 \leq small'$. The logic for that lemma is something along these lines: if $x \leq \e + x^2$, then either $x \leq O(\e)$ or $x \geq 1 - \e$. But in our case, $x = \alpha_P(w) \alpha_Q(w) / n^2$ cannot be close to $1$.}
\end{proof}

\subsection{Proofs of Lemmas}

We turn to the proofs of \cref{lem:q-2nd-moment}.

\begin{proof}[Proof of \cref{lem:q-2nd-moment}]
  Expanding $q(x)^2$, we see
  \begin{align*}
  q(x)^2 & = (\iprod{x,v}^2 - \iprod{x,v}\iprod{\mu_P,v} - \iprod{x,v}\iprod{\mu_Q,v} + \iprod{\mu_P,v}\iprod{\mu_Q,v})^2 \\
  & = \iprod{x,v}^4 - \iprod{x,v}^3 (\iprod{\mu_P,v} + \iprod{\mu_Q,v}) + \iprod{x,v}^2 \iprod{\mu_P,v}\iprod{\mu_Q,v} + \iprod{x,v}^2 (\iprod{\mu_P,v} + \iprod{\mu_Q,v})^2 \\
  & - \iprod{x,v} (\iprod{\mu_P,v} + \iprod{\mu_Q,v}) \iprod{\mu_P,v} \iprod{\mu_Q,v} + \iprod{\mu_P,v}^2 \iprod{\mu_Q,v}^2
  \end{align*}
  Taking the expectation under $\cN(0,\Sigma(w))$, the odd terms (with respect to $x$) vanish, leaving
  \begin{align*}
  \E_{x \sim \cN(0,\Sigma(w))} q(x)^2 & = \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^4 + \E_{x \sim \cN(0,\Sigma(w)} \iprod{x,v}^2 (\iprod{\mu_P,v} \iprod{\mu_Q,v} + (\iprod{\mu_P,v} + \iprod{\mu_Q,v})^2)\\
  & + \iprod{\mu_P,v}^2 \iprod{\mu_Q,v}^2
  \end{align*}
  As polynomials in $w$, we have the equality
  \[
  \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^4 = 3 (\E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2)^2\mper
  \]
  So, dropping some squares,
  \[
  \E_{x \sim \cN(0,\Sigma(w))} q(x)^2 \succeq 3 (\E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2)^2 + \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2 \iprod{\mu_P,v} \iprod{\mu_Q,v}\mper
  \]
  Since
  \[
  \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2 \iprod{\mu_P,v}\iprod{\mu_Q,v} \succeq - \E_{x \sim \cN(0,\Sigma(w))} \iprod{x,v}^2 (\iprod{\mu_P,v} - \iprod{\mu_Q,v}^2
  \]
  we are done.
\end{proof}


\begin{proof}[Proof of \cref{lem:p-norm-bounds}]
  \Snote{TODO: fill this in}
\end{proof}


==> separating-polynomials.tex <==
\section{Separating Polynomials}

In this section we prove \cref{lem:mean-separated,lem:variance-separated,lem:covariance-separated}.
The following facts will be useful.

\begin{fact}
\label[fact]{fact:var-f-squared}
  Let $P,Q$ be probability distributions on $\R$ such that $\E_{X \sim P} X = 1, \E_{X \sim Q} X = -1$, $\V(P),\V(Q) \leq \epsilon$, and $\E_{X \sim P} (X - 1)^4, \E_{X \sim Q} (X + 1)^4 \leq \epsilon$.
  Then $\V_{P/2 + Q/2}(X^2) \leq O(\epsilon)$.
\end{fact}
\begin{proof}
  We expand
  \begin{align*}
  \V_{P/2+Q/2}(X^2) & = \E_{P/2+Q/2} X^4 - (\E_{P/2+Q/2} X^2)^2
  \end{align*}
  By hypothesis, $\E_P X^2, \E_Q X^2 = 1 \pm \e$.
  Similarly, $\E_P X^4 - 1 = \E_P (X^2 - 1)(X^2 + 1) = \E_P (X-1)(X+1)(X^2+1) \leq O(\epsilon)$.
\end{proof}

\begin{fact}
\label[fact]{fact:fake-gaussian-to-norm}
  For any degree-$t$ polynomial $p$,
  \[
  \cA \proves{O(t)} \Paren{\E_{g \sim \cN(\mu(w),\Sigma(w))} p^2}^{16} \leq O(\|p\|)^{32}
  \]
\end{fact}
\begin{proof}
  By \cref{lem:emp-pop},
  \[
  \cA \proves{O(t)} \Paren{\E_{g \sim \cN(\mu(w),\Sigma(w))} p^2 }^2 \leq \Paren{\frac 2 n \sum_{i=1}^n w_i p(X_i')^2 }^2 + O_t(\delta) \Paren{\E_{g \sim \cN(\mu(w),\Sigma(w))} p^2}^2
  \]
  using \cref{fact:hypercontractivity}, which rearranges to
  \[
    \cA \proves{O(t)} \Paren{\E_{g \sim \cN(\mu(w),\Sigma(w))} p^2 }^2 \leq O\Paren{\frac 2 n \sum_{i=1}^n w_i p(X_i')^2 }^2
  \]
  Applying the same reasoning again with \cref{lem:moment-compare} gives the fact.
\end{proof}

\subsection{Mean Separation}

\Snote{TODO: $\e$ is overloaded here.}

\cref{lem:mean-separated} follows from the following facts.
The first is a straightforward exercise.

\begin{fact}
  Let $P,Q$ be univariate probability distributions with means $\mu_P, \mu_Q$ respectively.
  Then $f(X) = \tfrac 2 {\mu_P - \mu_Q} X - \tfrac{\mu_P + \mu_Q}{\mu_P - \mu_Q}$ has $\E_P f = 1, \E_Q f = -1$.
\end{fact}

\begin{fact}
  In the setting of \cref{lem:mean-separated}, with Gaussians $P,Q$ having $TV(P,Q) \geq 1 - \exp(-1/\epsilon)$,
  \[
  \V_P(f), \V_Q(f) \leq O \Paren{\frac 1 {\sqrt{\log(1/\epsilon)}}}\mper
  \]
\end{fact}
\begin{proof}
  We prove the fact for $\V_P(f)$; the argument for $\V_Q(f)$ is symmetric.
  We have
  \[
  \V_P(f) \leq O(1) \cdot \frac{\iprod{vv^\top,\Sigma_Q}}{\iprod{v,\mu_P - \mu_Q}^2} \leq O\Paren{\frac 1 {\sqrt{\log(1/\epsilon)}}}
  \]
  since $P,Q$ are mean separated.
\end{proof}

\begin{fact}
  In the setting of \cref{lem:mean-separated}, $\cA \proves{O(1)} (\E_w (f(X) - \mu_f)^2)^{16} \leq 1/\log(1/\epsilon)^{\Omega(1)}$.
\end{fact}
\begin{proof}
  By \cref{fact:var-f-squared}, $\V_{P/2+Q/2}(f^2) \leq 1/\log(1/\epsilon)^{\Omega(1)}$, so it will be enough to show that $\cA \proves{O(1)} (\E_w (f(X) - \mu_f)^2)^2 \leq O(\V_{P/2+Q/2}(f^2))$.

  It is an exercise to check that for indeterminates $a,b$,
  \[
  \proves{4}^{a,b} (\V_{g\sim \cN(0,1)} [ag+b])^2 \leq O(\V_{g \sim \cN(0,1)} [(ag+b)^2]) \mper
  \]
  Hence also for indetermintes $\mu,\sigma$,
  \begin{equation}\label{eq:linear-var-sq-1}
  \proves{4}^{a,b,\mu,\sigma} (\V_{g\sim \cN(\mu,\sigma^2)} [ag+b])^2 \leq O(\V_{g \sim \cN(\mu,\sigma^2)} [(ag+b)^2]) \mper
  \end{equation}

  Now, $\E_w (f(X) - \mu_f)^2 = \V_{\cN(\mu(w),\Sigma(w))} f$ by definition.
  Using \eqref{eq:linear-var-sq-1},
  \[
  \cA \proves{O(1)} (\E_w (f(X) - \mu_f)^2)^2 \leq O(\V_{\cN(\mu(w),\Sigma(w))} f^2)\mper
  \]
  \Snote{TODO: this is terrible. actually prove this.} Using similar reasoning as in \cref{fact:fake-gaussian-to-norm}, $\cA \proves{O(1)} (\E_{\cN(\mu(w),\Sigma(w))} f^2 )^{16} = 1 \pm (\delta + \epsilon)^{\Omega(1)}$, and so by applying \cref{fact:fake-gaussian-to-norm} a second time, we find can conclude that
  \[
  \cA \proves{O(1)} (\E_w (f(X) - \mu_f)^2)^{16} \leq O_{\delta,\epsilon}(\V_{P/2+Q/2}(f^2))\mper
  \]
\Snote{TODO: redo this proof substantially. need some better primitives to compare variances under different distributions.}
\end{proof}

\subsection{Covariance Separation}

The key fact for the proof of \cref{lem:covariance-separated} is the following.

\begin{fact}
\label[fact]{fact:sos-quadratic-variance}
  Let $F(x_1,\ldots,x_d)$ be a symbolic quadratic polynomial.
  Then
  \[
  \proves{O(1)}^{F} \V_{\cN(0,I)}(F)^2 \leq O(\V_{\cN(0,I)}(F^2))\mper
  \]
\end{fact}
\begin{proof}
  We represent $F$ in the Hermite basis, writing $F(x) = Q(x) + L(x) + C$ where $Q$ is a linear combination of degree-$2$ Hermite polynomials (the coefficients of said linear combination still being indeterminates), $L$ is a linear combination of degree-$1$ Hermite polynomials, and $C$ is a symbolic degree-$0$ polynomial (i.e. a single indeterminate representing the constant term in $F$).
  To begin, as polynomials in the coefficients of $F$,
  \begin{equation}
    \label{eq:var-F}
    \V F = \E F^2 - C^2 = \E Q^2 + \E L^2\mper
  \end{equation}
  Let $A$ be the matrix of indeterminates such that $Q(x) = x^\top A x - \tr(A)$.
  Then one may verify the identities
  \begin{align}
    \label{eq:EF4}
      \E[F^4] & = \E[Q^4] + 6 \E[Q^2L^2] + 6 C^2 \E[Q^2]\\
      & + 12 C \E[QL^2] + \E[L^4] + 6 C^2 \E[L^2]+C^4\\
      & = 3\E[Q^2]^2 + c \Tr(A^4) + 6 \E[Q^2L^2] + 6 C^2 \E[Q^2]\\
      & + 12 C \E[QL^2] + 3 \E[L^2]^2 + 6 C^2 \E[L^2] + C^4
  \end{align}
  for some universal constant $c > 0$, as polynomials in the coefficients of $Q, L,C$.
  Hence
  \begin{align*}
  \V[F^2] & = \E [F^4] - (\E[F^2])^2\\
  & = 3\E[Q^2]^2 + c \Tr(A^4) + 6 \E[Q^2L^2] + 6 C^2 \E[Q^2]\\
      & + 12 C \E[QL^2] + 3 \E[L^2]^2 + 6 C^2 \E[L^2] + C^4 \\
      & - \E[Q^2]^2 - 2 \E[Q^2] \E[L^2] - 2 C^2\E[Q^2] - \E[L^2]^2 - 2 \E[L^2 C^2] - C^4 \\
      & = 2 \E[Q^2]^2 + c \Tr(A^4) + 6 \E[Q^2 L^2] + 4 C^2 \E[Q^2] \\
      & + 12 C \E [QL^2] + 2 \E[L^2]^2 + 4 C^2 \E[L^2] - 2 \E[Q^2] \E[L^2] \\
      & \succeq \E[Q^2]^2 + \E[L^2]^2 + 6 \E[Q^2 L^2] + 4 C^2 \E[Q^2] + 12 C \E[QL^2] + 4 C^2 \E[L^2]
  \end{align*}
  where in the last step we used $c \Tr A^4 \succeq 0$ and $-2\E[Q^2]\E[L^2] \preceq \E[Q^2]^2 + \E[L^2]^2$.
  This is nearly equal to $(\V F)^2$ added to a sum-of-squares polynomial, but for the presence of the term $12 C \E [QL^2]$.
  We bound that term by splitting it into parts.
  First of all,
  \[
  4 \sqrt{6} C \E Q L^2  = \E L^2 \cdot 2 (\sqrt{6} \cdot Q)(2C) \preceq 6 \E L^2 Q^2 + 4 C^2 \E L^2\mper
  \]
  Note that $12 - 4 \sqrt{6} \leq 2.3$, and
  \[
  2.3 C \E QL^2 = \E 2 \cdot ( (2 C Q) (\tfrac{2.3}{4} L^2)) \preceq 4 C^2 \E Q^2 + (2.3/4)^2 \E L^4 \preceq 4 C^2 \E Q^2 + 0.999 \E[L^2]^2\mper
  \]
  So all together, we obtained
  \[
    \E[Q^2]^2 + \E[L^2]^2 + 6 \E[Q^2 L^2] + 4 C^2 \E[Q^2] + 12 C \E[QL^2] + 4 C^2 \E[L^2] \preceq 0.0001( \E[Q^2]^2 + \E[L^2]^2) \preceq \Omega(\V F)^2\mper
  \]
\end{proof}

Now we can prove \cref{lem:covariance-separated}.

\begin{proof}[Proof of \cref{lem:covariance-separated}]
  It is easy to check $\E_P f = 1, \E_Q f = -1$.
  Next we bound $\V_P f, \V_Q f$.
  Let $h(X) = \iprod{Y, (I - \Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2}) Y}$.
  It will be enough to show that $\V_P h, \V_Q h \leq ?? \cdot \|I - \Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2} \|_F^2$.

  Beginning with $\V_P h$, a calculation yields
  \[
  \E_P h^2 = \E_{\cN(0,I)} \iprod{x, (I - A)x}^2 + 4 \| (I-A) v\|^2 - (\E_{\cN(0,I)} \iprod{x, (I-A) x})^2
  \]
  where $A = \Sigma_P^{-1/2} \Sigma_Q \Sigma_P^{-1/2}$ and $v = \tfrac 12 \Sigma_P^{-1/2} (\mu_P - \mu_Q)$.
  Since $\Sigma_P$ $\e$-approximates $\Sigma_Q$ in PSD order and we may assume mean separation (case 1 of \cref{lem:gaussian-cases}) does not hold, it follows that $\|v\| \leq O( \e^{-1} \sqrt{\log(1/\epsilon)})$.
  So $\|(I-A)v\|^2 \leq \tilde{O}(\|I-A\|_F^2 /\e^2)$.
  A straightforward calculation using moments of $\cN(0,I)$ shows that the remaining term $\E_{\cN(0,I)} \iprod{x, (I - A)x}^2 + 4 \| (I-A) v\|^2 - (\E_{\cN(0,I)} \iprod{x, (I-A) x})^2$ is also bounded as $O(\|I-A\|_F^2)$.

  The case of $\V_Q h^2$ is similar, using in place of the bound on $\|I - A\|_F^2$ that $\|\Sigma_Q^{1/2}\Sigma_P^{-1/2}(I-A) \Sigma_P^{-1/2} \Sigma_Q^{1/2}\|$ is equal to
  \[
  \Tr A(I-A)A (I-A) \leq \e^{-2} \|I-A\|_F^2
  \]
  since $\Sigma_P,\Sigma_Q$ $\e$-approximate each other in PSD order.
  This completes our verification of point (2) in the hypothese of \cref{lem:cluster}.

  Point (3) follows from hypercontractivity of Gaussians.

  Finally, (4) follows from \cref{fact:var-f-squared} and \cref{fact:sos-quadratic-variance}.
\end{proof}



\subsection{Variance Separation}


Then if you have $P, Q$ where $\iprod{v, \Sigma_Qv} \leq \eps$ and $\iprod{v, \Sigma_Pv} = 1$, we see that an application of the moment-comparison lemma implies
\[ \cA \proves{} (\alpha_P \E_P[\iprod{X, v}^2] + \alpha_Q \E_Q[\iprod{X, v}^2])^8 - (\eps + \delta) \E_{P/2 + Q/2}[\iprod{X, v}^4]^4 - \alpha_P^{80} \alpha_Q^{80} \Var_{P, Q}[\iprod{X,v}^2]^4 \leq \E_w[\iprod{X, v}^2]^8   \] 

Using the fact that if $a, b  > 0$ then $(a+b)^8 \geq a^8 + b^8$, and hypercontractivity of $P$ and $Q$, and the fact that $\iprod{\mu_P, v}^2 \leq \eps^2$ and $\iprod{\mu_Q, v}^2 \leq \eps^2$, we see

\[ \cA \proves{} \E_w[\iprod{X, v}^2]^8 \geq (\alpha_P^8 - \alpha_P^{9} - \eps - \delta) \E_P[\iprod{X,v}^2]^8 \geq (\alpha_P^7 \alpha_Q - \eps - \delta) \Var_P[\iprod{X,v}]^8\]

Similarly we have the following inequality for $q_w(x)$.
\[ 
\cA\proves{} \E_w[q_\eps(x)]^8 \geq (\alpha_P \E_P[q_\eps(x)] + \alpha_Q \E_Q[q_{\eps}(x)])^8 - (\eps + \delta) (\E_P[q^2_\eps(x)] + \E_Q[q^2_\eps(x)])^4 - \alpha_P^{80} \alpha_Q^{80} \Var_{P, Q}[q_\eps(x)]^4
\]
Collecting terms similar to before, and using the fact that $(\E[q_{\eps}(x)^2] - \E[q_{\eps}(x)]^2)^2 \leq O(\eps^{\Omega(1)})$

\[ 
\cA \proves{} \E_w[q_\eps(x)]^{16} \geq (\alpha_Q^{16} \alpha_P^2 - \eps - \delta)\E_Q[q_{\eps}(x)]^{16}
\]

We now use the following property of $q_{\eps}$, that $\sigma^2 \E_{\cN(\eps, \sigma)}[q_\eps(x)]^2 \leq O(\eps^2)$. Combining these together and using the fact that $\iprod{v, \Sigma_Qv} \leq \eps$ we get 

\[ \cA \proves{} O(\eps^2) \geq \alpha_Q^{16} \alpha_P^8 \E_Q[q_{\eps}(x)]^{16}
\E_P[\iprod{X,v}^2]^8 \geq  \alpha_Q^{16} \alpha_P^{16}\]


The following fact will be useful 
	\begin{fact}
	There is a polynomial $q$ of degree $d < O\left(\frac{L\log^2(1/\delta)}{\delta}\right)$ satisfying the following properties.
	\begin{enumerate}
		\item $q(x) \in [0, \delta]$ for $x \in [t, L] \cup [L, t]$.
		\item $q(x) \in [1, 1+ \delta]$ for $x \in [-L, L]$.
		\item $q(x) \in [0, 1+ \delta]$ for $x \in [-L-3\delta, -L-\delta]\cup[L+\delta, L+3\delta]$.
		\item $|q(x)| < 4 \cdot (4x)^{t}$ for $|x| > 1$
	\end{enumerate}
\end{fact} 
\begin{proof} 
	We will use the following Theorem from ~\cite{DGJSV09}. 
	\begin{fact}[Theorem 3.5 in ~\cite{DGJSV09}]
		\label{fact:boxpoly}
		Let $0 < \eta < 0.1$, then there exist constants $C, c$ such that for 
		\[ a:= \eta^2 / C\log(1/\eta)\text{ and }K = 4c\log(1/\eta)/a + 2 < O(\log^2(1/\eta)/\eta^2)\]
		there is a polynomial $p(t)$ of degree $K$ satisfying 
		\begin{enumerate}
			\item $p(t) > \sign(t) > -p(-t)$ for all $t \in \mathbb{R}$.
			\item $p(t) \in [\sign(t), \sign(t) + \eta]$ for $t \in [-1/2, -2a] \cup [0, 1/2]$.
			\item $p(t) \in [0, 1+\eta]$ for $t \in (-2a, 0)$
			\item $|p(t)| \leq 2 \cdot (4t)^K$ for all $t > \frac{1}{2}$. 
		\end{enumerate}
	\end{fact}
	Let $p(x)$ be the degree $d < O\left(\frac{L\log^2(1/\delta)}{\delta}\right)$ polynomial from Fact~\ref{fact:boxpoly}. We now construct a polynomial $q(x)$ that will be close to $0$ in the range $[1, L]$ and $[-L, -1]$ and close to $1$ in the range $[-1, 1]$. 
	\[
	q(x) = p\left(t+\frac{x}{4L}\right) + p\left(-t+ \left(1+\frac{x}{4L} \right) \right) - 1
	\]
\end{proof} 

We now move to the construction of $f$. Observe first, that for any $D = \cN(\mu, \sigma)$ wtih $\mu < \eps^2 \sqrt{\log(1/\eps)}$ and $\sigma \leq 1$ we can rescale the polynomial $q$ from Fact~\ref{fact:boxpoly} to be $q'$, which is $\eps$-close to $1$ whenever $|x| \in [0, \eps]$ and $\eps$-close to $0$ whenever $|x| \in [2\eps, 1/\eps^2]$. 
We prove upper and lower bounds on $\E_{\cN(\mu, \sigma)}[q'(x)]$.
\begin{align*}
\sigma \E_{\cN(\mu, \sigma)}[q(x)] &= \Theta \left(\int_{|x| \in [\eps, 1/\eps^2]} q'(x) \exp(-(x-\mu)^2/2\sigma^2)  dx + \int_{|x| \in [0, \eps]} q'(x) \exp(-(x-\mu)^2/2\sigma^2)  dx \right)  \\
&+ \Theta \left( \int_{|x| > 1/\eps^2} q'(x) \exp(-(x-\mu)^2/2\sigma^2)  dx \right) 
\end{align*}
Each integral above may be bounded as follows
\begin{equation}
0 \leq \int_{|x| \in [\eps, 1/\eps^2]} q'(x)  \exp\left(-(x-\mu)^2/2\sigma^2 \right) dx \leq O\left( \sigma \Pr_{\cN(\mu, \sigma)}[|x| \in [1, L]] \cdot \eps \right) \leq O(\sigma \eps)
\end{equation}
For the second term, observe that 
\begin{equation}
\sigma \Pr[|x| \in [0, \eps]] \cdot 1\leq \int_{[0, \eps]} q'(x) \exp(-(x-\mu)^2/2\sigma^2) dx \leq \sigma \Pr[|x| \in [0, \eps]] \cdot (1+\eps)
\end{equation}
Since $c_0 \eps \geq \sigma \Pr_{\cN(\mu, \sigma)}[|x| \in [0, \eps]] \geq c_1 \eps$ for some constants $c_0, c_1$, we get 
\begin{equation}
\eps c_0 \cdot 1\leq \int_{|x| \in [0, \eps]} q(x) \exp(-(x-\mu)^2/2\sigma^2) dx \leq \eps c_1 \cdot (1+\delta)
\end{equation}
and finally, using the following lemma from \cite{KKK19}
\begin{lemma}[Tail Integral] \label{lem:tail-estimate}
	\[\int_{[1/\eps^3, \infty]} \exp\left(-\frac{x^{2}}{C}\right) x^{2d}  dx < \exp\left(-\frac{L^{2}}{C}\right) ((L)^{4d} + (16d)^{d}) \mper \]
\end{lemma}
Substituting the values above and taking integrals gives us 
\begin{equation}
0 \leq \int_{|x| > 1/\eps^2} q(x) \exp(-(x-\mu)^2/2\sigma^2) dx \leq \eps \sigma 
\end{equation}
Adding the above equations up, we see
\begin{equation}
c_0 \eps \leq \sigma \cdot \E_{\cN(\mu, \sigma)}[q(x)] \leq  c_1 \eps + O(\sigma \eps)
\end{equation}

We now use this to define a function $g$ that almost satisfies the right properties, which after scaling give us our $f$. WLOG let $\eps \iprod{v, \Sigma_P v} > \iprod{v, \Sigma_Q v}$, and define $g(\iprod{X,v})$ to be 
\[ g(\iprod{X,v}) := q \left( \frac{\iprod{X, v} - (1/2)\iprod{\mu_P + \mu_Q, v}}{10 \iprod{v, \Sigma_P v}} \right). \]
$\E_P[g(\iprod{X,v})] \leq \E_{Z \sim \cN(\eps^2 \sqrt{\log(1/\eps)}, 1)}[q(Z)] \leq c_1 \eps + \eps$ and $\E_Q[g(\iprod{X,v})] \geq \E_{Z \sim \cN(\eps^2\sqrt{\log(1/\eps)}, \eps)}[q(Z)] \geq c_0 \eps$ and so as long as $O(\eps) < c_0/2$, $\E_P[g(\iprod{X,v})] - \E_Q[g(\iprod{X,v})] \geq c_0/2$. Additionally since $q(x)$ is $[0, \eps]$ for $1-\eps$ of the mass of $P$ and $[1,1+\eps]$ for $1-\eps$ of the mass of $q$, with the remaining integrals being appropriately bounded we see that the variance is at most $O(\eps^2)$. 
\[ f(\iprod{X,v}) = \frac{ \left( 2g(\iprod{X,v}) - \E_P[g(\iprod{X,v})] - \E_Q[g(\iprod{X,v})] \right)}{\E_P[g(\iprod{X,v})] - \E_Q[g(\iprod{X,v})]} \]
This will satisfy $\E_P[f] = 1$ and $\E_Q[f] = -1$, since the scaling is by constants, the variance being $O(\eps)$. 


==> variance-separated.tex <==
\section{Variance-Separated Case}

In this section we prove the following lemma.

\begin{proof}[Proof of \cref{lem:var_sep}]

\cref{lem:fake_var_lowerbound} implies, 
\begin{align}
\cA &\proves{O(1)} \iprod{v, \Sigma(w)v}^{4d} \\
&\geq \Big[ \Omega(1 ) \cdot \Paren{\xi \cdot \iprod{v, \Sigma_a v} }^{4} \cdot \Brac{ (\alpha_a(w)/n)^{4} - \xi  }^{2} + \Omega(1) \cdot \Paren{\xi \cdot \iprod{v, \Sigma_b v} }^{4} \cdot \Brac{ (\alpha_b(w)/n)^4  - \xi }^{2} \\
&\qquad - O(1) \cdot \eps \cdot m_{a, b} \Big]^d\\
&\geq \Big[ \Omega(1 ) \cdot \Paren{\xi^2 \cdot \iprod{v, \Sigma_a v}  \iprod{v, \Sigma_b v}}^{2} \cdot \Brac{ (\alpha_a(w)/n)^{4} - \xi  } \cdot \Brac{ (\alpha_b(w)/n)^4  - \xi } \\
&\qquad - O(1) \cdot \eps \cdot m_{a, b} \Big]^d\\
\end{align}
An application of \cref{lem:fake_var_upperbound} implies 

\begin{align}
\cA &\proves{}  \iprod{v, \Sigma_a v}^{4d}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \iprod{v, \Sigma(w)v}^{4d} 
\end{align}

The above together imply 
\begin{align}
\cA &\proves{}  \frac{\iprod{v, \Sigma_a v}^{4d}}{\Paren{\xi^2 \cdot \iprod{v, \Sigma_a v}  \iprod{v, \Sigma_b v}}^{2d}}\\
&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \\
&\qquad \cdot \Brac{ \Omega(1 ) \cdot \Brac{ (\alpha_a(w)/n)^{4} - \xi  } \cdot \Brac{ (\alpha_b(w)/n)^4  - \xi } - \frac{\eps \cdot m_{a, b}}{\Paren{\xi^2 \cdot \iprod{v, \Sigma_a v}  \iprod{v, \Sigma_b v}}^{2}} }^d\\
\end{align}

%
%Rearranging these, we get
%\begin{align}
%\cA &\proves{}  \frac{\iprod{v, \Sigma_a v}^{4d}}{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^d}\\
%&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
%\end{align}
%We repeat the above argument for $b$ to get 
%
%\begin{align}
%\cA &\proves{}  \frac{\iprod{v, \Sigma_b v}^{4d}}{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^d}\\
%&\geq \exp(-O(d))\Brac{ (\alpha_b(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{2d}
%\end{align}
%
%Combining these, we get 
%
%\begin{align}
%\cA &\proves{}  \frac{\iprod{v, \Sigma_b v}^{8d} +\iprod{v, \Sigma_b v}^{8d} }{\Big[\Paren{ \iprod{\mu_a - \mu_b, v} - \sqrt{\log(1/\xi)} \Paren{ \sqrt{\iprod{v, \Sigma_a v}} + \sqrt{\iprod{v, \Sigma_b v} } } }^8 - \eps \cdot  m_{a, b} \Big]^{2d}}\\
%&\geq \exp(-O(d))\Brac{ (\alpha_a(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2\Brac{ (\alpha_b(w)/n)^4 - O(\tau^4)  - (\delta + \eps) \exp(\tilde{O}(d))}^2 \\
%&\qquad \cdot \Brac{(1/n)^4 (\alpha_a(w) \alpha_b(w))^2 - \xi }^{4d}
%\end{align}
%
%
%
%WLOG let $\iprod{v, \Sigma_a v} > \iprod{v, \Sigma_b v}$, then for any $a, b$ such that $G_a, G_b$ are $\eps^4$-variance separated, there is a $v \in \R^d$ such that 
%
%\begin{equation}~\label{eqn:var_sep}
%\iprod{v, \Sigma_a v} \leq \frac{\iprod{v, \Sigma_b v}}{\eps^4}	
%\end{equation}
%		
%\cref{lem:fake_var_lowerbound} and equation~\ref{eqn:mean_sep}, and the fact that $\proves{} a^2 + b^2 \geq 2 ab$ implies, 
%\begin{align}
%\cA &\proves{O(1)} \iprod{v, \Sigma(w)v}^4 \\
%&\geq \Omega (1) \cdot \Paren{ \Paren{\frac{k}{n}}^4 \alpha_a(w)^2 \alpha_b(w)^2 \iprod{\mu_a - \mu_b, v}^8 + \frac{k^2}{n^2} \alpha_b(w)^2 \Iprod{v, \Sigma_a v}^4 + \frac{k^2}{n^2} \alpha_a(w)^2 \Iprod{v,  \Sigma_b v}^4 } \\
%&\geq \Omega (1) \cdot \Paren{ \frac{k^2}{n^2} \alpha_b(w)^2 \Iprod{v, \Sigma_a v}^4 + \frac{k^2}{n^2} \alpha_a(w)^2 \Iprod{v,  \Sigma_b v}^4 }\\
%&\geq \Omega (1) \cdot \Paren{ \frac{k^2}{n^2} \alpha_a(w) \alpha_b(w) \Iprod{v, \Sigma_a v}^2 \Iprod{v,  \Sigma_b v}^2 }\\
%&\geq \frac{\Omega(1)}{\eps^4} \cdot \Paren{ \frac{k^2}{n^2} \alpha_a(w) \alpha_b(w) \Iprod{v,  \Sigma_b v}^4 }\label{eq:var_sep_lb}
%\end{align}
%An application of \cref{lem:fake_var_upperbound} to equation~\ref{eq:mean_sep_lb} raised to the $d^{th}$ power implies 
%
%\begin{align}
%\cA &\proves{O(d)}  \Paren{ 1 + \eps^2 \exp(d) }\iprod{v, \Sigma_b v}^{4d} \geq \Paren{\Omega(1) - \eps \exp(d)} \cdot \iprod{v, \Sigma(w)v}^{2d} \\
%&\geq \Paren{\Omega(1) - \eps \exp(d)} \Paren{ \frac{\Omega(1)}{\eps^4} \cdot \Paren{ \frac{k^2}{n^2} \alpha_a(w) \alpha_b(w) \Iprod{v,  \Sigma_b v}^4 } }^d
%\end{align}
%Rearranging, 
%\begin{align}
%\cA &\proves{}  O(\eps)^{32d} \cdot \Paren{ 1 + \eps^2 \exp(d) } \geq \Paren{\Omega(1) - \eps \exp(d)} \cdot \Paren{ \Paren{\frac{k}{n}}^{2} \cdot \alpha_a(w) \alpha_b(w) }^d
%\end{align}
%Let $\eps_0$ be the constant below which robust recovery is possible as per \SKnote{cite}. Then, setting $\eps$ and $\tau$ small enough in terms of this constant, we see 
%
%\begin{align}
%\cA &\proves{}  O(\eps)^{32d} \geq \Paren{ \Paren{\frac{k}{n}}^{2} \cdot \alpha_a(w) \alpha_b(w) }^d
%\end{align}


\end{proof}

%\begin{lemma}
%  \label[lemma]{lem:var-lb}
%  In the setting of \cref{lem:var-sep-main}, there is a constant $c > 0$ such that for every $i \in [k]$,
%  \[
%  \cA \proves{t} \iprod{v,\Sigma(w) v}^4 \geq ??
%  \]
%\end{lemma}
%\begin{proof}
%  We begin by expanding the definition
%  \[
%    \iprod{v,\Sigma(w)v} = \frac 1 {2n} \sum_{i \in [n]} w_i \iprod{X_i' - X_j',v}^2
%  \]
%
%  \Snote{working here, march 22}
%  
%\end{proof}

